SEEV: Synthesis with Efficient Exact Verification for ReLU Neural Barrier Functions

Neural Control Barrier Functions (NCBFs) have shown significant promise in enforcing safety constraints on nonlinear autonomous systems. State-of-the-art exact approaches to verifying safety of NCBF-based controllers exploit the piecewise-linear structure of ReLU neural networks, however, such approaches still rely on enumerating all of the activation regions of the network near the safety boundary, thus incurring high computation cost. In this paper, we propose a framework for Synthesis with Efficient Exact Verification (SEEV). Our framework consists of two components, namely (i) an NCBF synthesis algorithm that introduces a novel regularizer to reduce the number of activation regions at the safety boundary, and (ii) a verification algorithm that exploits tight over-approximations of the safety conditions to reduce the cost of verifying each piecewise-linear segment. Our simulations show that SEEV significantly improves verification efficiency while maintaining the CBF quality across various benchmark systems and neural network structures. Our code is available at https://github.com/HongchaoZhang-HZ/SEEV.

==> sections/Detailed.tex <==
\section{Verification Algorithm}
\label{sec:verification}
In this section, we present our proposed approach to verifying safety.

\subsection{Branch-and-Bound Formulation and Algorithm}
\label{subsec:BaB}
The key insight of our approach is that the constraints of (\ref{eq:convex-relaxation-opt}) are determined by the sets of neurons $S(x)$ and $T(x)$. Hence, if these sets are fixed, then the optimization problem can be simplified. Formally, we define $\mathcal{Q} = (\mathcal{P}, \mathcal{Z}, \mathcal{N}, \mathcal{U})$, where $\mathcal{P}$, $\mathcal{Z}$, $\mathcal{N}$, and $\mathcal{U}$ are subsets of $\{1,\ldots,L\} \times \{1,\ldots,M_{i}\}$ (i.e., neurons) whose pre-activation inputs are positive, zero, negative, and undetermined, respectively. We let $\mathcal{X}(\mathcal{Q})$ denote the set of states that are consistent with $\mathcal{Q}$, so that $x \in \mathcal{X}(\mathcal{Q})$ if and only if
\begin{equation}
\label{eq:define-X-Q}
z_{j}^{i} \left\{
\begin{array}{ll}
> 0, & (i,j) \in \mathcal{P} \\
= 0, & (i,j) \in \mathcal{Z} \\
< 0, & (i,j) \in \mathcal{N} \\
\in \mathbb{R}, & (i,j) \in \mathcal{U}
\end{array}
\right.
\end{equation}
The idea of the branch-and-bound algorithm is to solve sub-problems that attempt to bound the solutions of (\ref{eq:convex-relaxation-opt}) when $x \in \mathcal{X}(\mathcal{Q})$ for some value of $\mathcal{Q}$. For a fixed value of $\mathcal{Q}$, (\ref{eq:convex-relaxation-opt}) reduces to
\begin{equation}
        \label{eq:opt-fixed-evaluation}
    \begin{array}{ll}
    \mbox{minimize} & v^{T}f(x) \\
    \mbox{s.t.} & v \in \mathcal{V}(\mathcal{Q}) \\
    & v^{T}g(x) = 0 \\
    & b(x) = 0 \\
    & x \in \mathcal{X}(\mathcal{Q})
    \end{array}
\end{equation}
where $\mathcal{V}(\mathcal{Q}) = \bigcup_{x \in \mathcal{X}(\mathcal{Q})}{\mathcal{V}(x)}$. A branch-and-bound algorithm that verifies an NCBF by solving subproblems of the form (\ref{eq:opt-fixed-evaluation}) is given as Algorithm \ref{algo:BaB}. The algorithm returns $1$ if the NNCBF feasibility has been verified and $0$ if the feasibility check fails.

%  \begin{center}
% \begin{algorithm}[]
% 	\caption{Branch-and-bound algorithm for NNCBF verification (BaB\_VERIFY).}
% 	\label{algo:BaB}
% 	\begin{algorithmic}[1]
%         \STATE \textbf{Input:} Set $\mathcal{Q} = (\mathcal{P},\mathcal{Z}, \mathcal{N}, \mathcal{U})$
% 		%\STATE Initialize $\mathcal{Q} \leftarrow (\mathcal{P}, \mathcal{Z}, \mathcal{N}, \mathcal{U})$
%             \STATE $opt\_val \leftarrow \mbox{optimal value of (\ref{eq:opt-fixed-evaluation}) with } \mathcal{Q}$
%             \IF{$opt\_val \geq 0$}
%              \RETURN $1$
%             \ELSE
%                 \IF{$\mathcal{U} == \emptyset$}
%                 \RETURN EXACT\_VERIFY($\mathcal{P}$, $\mathcal{Z}$, $\mathcal{N}$)
%                 \ENDIF
%                 \STATE $(i,j) \leftarrow$ NEURAL\_SPLIT($\mathcal{P}$, $\mathcal{Z}$, $\mathcal{N}$, $\mathcal{U}$) 
%                 \STATE $p_{1} \leftarrow \mbox{BaB-VERIFY}(\mathcal{P} \cup \{(i,j)\}, \mathcal{Z}, \mathcal{N}, \mathcal{U} \setminus \{(i,j)\})$ 
%                 \STATE $p_{2} \leftarrow \mbox{BaB-VERIFY}(\mathcal{P}, \mathcal{Z} \cup \{(i,j)\}, \mathcal{N}, \mathcal{U} \setminus \{(i,j)\})$
%                 \STATE $p_{3} \leftarrow \mbox{BaB-VERIFY}(\mathcal{P}, \mathcal{Z}, \mathcal{N} \cup \{(i,j)\}, \mathcal{U} \setminus \{(i,j)\})$
%                 \IF{$p_{l}==1$ for $l=1,2,3$}
%                 \RETURN 1
%                 \ELSE
%                 \RETURN 0
%                 \ENDIF
%             \ENDIF
%         \end{algorithmic}
%         \end{algorithm}
% \end{center}
The idea of the algorithm is to attempt to verify safety by solving the optimization problem (\ref{eq:opt-fixed-evaluation}). If the safety condition fails, i.e., the value of the optimization problem is negative, the algorithm attempts to refine the solution by reducing the number of undetermined neurons.  The NEURAL\_SPLIT subroutine selects a neuron $(i,j)$ and the algorithm is run recursively on three sub cases, namely $(i,j) \in \mathcal{P}$, $(i,j) \in \mathcal{Z}$, and $(i,j) \in \mathcal{N}$. Neural splitting is a well-studied approach to neural network verification, and hence a variety of algorithms exist for selecting $(i,j)$. On the other hand, we note that none of these algorithms is designed specifically for NNCBF verification, and hence developing such an algorithm is a promising direction of future research.

If the set of undetermined neurons is empty, then we check safety using an exact algorithm; one such algorithm based on sum-of-squares optimization is given in \textbf{*ref NeurIPS}. We next turn to the initialization of $\mathcal{Q}$ as well as techniques for addressing each of the constraints of (\ref{eq:opt-fixed-evaluation}). 

\subsection{Solving the Sub-Problems}
\label{subsec:sub-problem}

In what follows, we discuss different aspects of Algorithm \ref{algo:BaB} including how to solve each sub-problem (\ref{eq:opt-fixed-evaluation}). As a starting point, we assume that (possibly loose) lower and upper bounds on $z_{j}^{i}$, denoted $\underline{\alpha}_{ij}$ and $\overline{\alpha}_{ij}$, respectively, have been computed. These bounds can be computed, for example, using interval bound propagation.

\subsubsection{Initialization:} We initialize $\mathcal{Q}$ using the bounds $\underline{\alpha}$ and $\overline{\alpha}$. We initially set $\mathcal{P} = \{(i,j) : \underline{\alpha}_{ij} > 0\}$, $\mathcal{Z} = \emptyset$, $\mathcal{N} = \{(i,j): \overline{\alpha}_{ij} < 0\}$, and $\mathcal{U} = \{(i,j) : \underline{\alpha}_{ij} \leq 0 \leq \overline{\alpha}_{ij}\}$. 

\subsubsection{Constraint $v \in \mathcal{V}(\mathcal{Q})$:} This constraint is applied element-wise to each $v_{j}^{i}$ as follows. If $i=1$, then $v_{j}^{1} = W_{1j}$. Otherwise, we apply the constraints
\begin{eqnarray*}
v_{j}^{i} &\geq& -\sum_{(i-1,j^{\prime}) \in \mathcal{U} \cup \mathcal{Z}}{W_{ijj^{\prime}}v_{j^{\prime}}^{i-1}} + \sum_{(i-1,j^{\prime}) \in \mathcal{P}}{W_{ijj^{\prime}}v_{j^{\prime}}^{i-1}} \\
v_{j}^{i} &\leq& \sum_{(i-1,j^{\prime}) \in \mathcal{U} \cup \mathcal{Z}}{W_{ijj^{\prime}}v_{j^{\prime}}^{i-1}} + \sum_{(i-1,j^{\prime}) \in \mathcal{P}}{W_{ijj^{\prime}}v_{j^{\prime}}^{i-1}} \\ 
v &\geq & -\sum_{(L,j^{\prime}) \in \mathcal{U} \cup \mathcal{Z}}{\beta_{Lj^{\prime}}\Omega_{j^{\prime}}v_{j^{\prime}}^{L}} + \sum_{(L,j^{\prime}) \in \mathcal{P}}{\Omega_{j^{\prime}}v_{j^{\prime}}^{L}} \\
v &\leq& \sum_{(L,j^{\prime}) \in \mathcal{U} \cup \mathcal{Z}}{\beta_{Lj^{\prime}}\Omega_{j^{\prime}}v_{j^{\prime}}^{L}} + \sum_{(L,j^{\prime}) \in \mathcal{P}}{\Omega_{j^{\prime}}v_{j^{\prime}}^{L}}
\end{eqnarray*}
We note that, if $(i,j) \in \mathcal{N}$, then the corresponding variables $v_{j}^{i}$ can be omitted since they do not affect the final computation of $v$. \textbf{Ideally we would like to develop a linear approximation of v (analogous to CROWN) so that the size of the optimization problem does not grow in the number of neurons.}

\subsubsection{Constraint $v^{T}g(x) = 0$:} This constraint is linear in the special case where the $g(x) = G$ for all $x$. Otherwise, we can use Lipschitz coefficients to relax to a linear constraint.

\subsubsection{Constraint $x \in \mathcal{X}(\mathcal{Q})$:} In order to ensure that this constraint is satisfied, we need $z_{j}^{i} > 0$ for all $(i,j) \in \mathcal{P}$,  $z_{j}^{i} = 0$ for all $(i,j) \in \mathcal{Z}$, and $z_{j}^{i} < 0$ for all $(i,j) \in \mathcal{N}$. In order to capture dependencies on the previous layer, we can introduce variables representing the post-activation outputs $\hat{z}_{j}^{i}$ and develop linear relaxations for the nonlinear relation $\hat{z}_{j}^{i} = \sigma(z_{j}^{i})$. Specifically, we can set $\hat{z}_{j}^{i} = 0$ for $(i,j) \in \mathcal{N} \cup \mathcal{Z}$, $\hat{z}_{j}^{i} = z_{j}^{i}$ for $(i,j) \in \mathcal{P}$, and $$z_{j}^{i} \leq \hat{z}_{j}^{i} \leq \frac{\overline{\alpha}_{ij}}{\overline{\alpha}_{ij}-\underline{\alpha}_{ij}}(z_{j}^{i}-\underline{\alpha}_{ij})$$ for $(i,j) \in \mathcal{U}$. Tighter approximation bounds from the literature can also be applied here.

%While each $z_{j}^{i}$ is a nonlinear function of the $z^{i-1}$ elements, these constraints can be relaxed by introducing variables representing the post-activation outputs $\hat{z}_{j}^{i}$. 


\subsubsection{Constraint $b(x) = 0$:} This constraint is equivalent to $\Omega^{T}\hat{z}^{L} + \psi = 0$.




\subsubsection{Objective Function:} The objective function is nonconvex. One relaxation would be to incorporate a bound on the Lipschitz coefficient of $f$. The approach would be to compute $L_{f}$ such that $||f(x)-f(x_{0})||_{1} \leq L_{f}||x-x_{0}||_{1}$, compute $x_{0}$ and $\rho > 0$ such that $$\mathcal{Q}(\mathcal{X}) \subseteq B_{1}(x_{0},\rho)$$ (the 1-norm ball centered at $x_{0}$), and then relax the objective function as $$v^{T}f(x) \geq v^{T}f(x_{0}) - ||v||_{\infty}\rho L_{f}.$$ Eq. (\ref{eq:opt-fixed-evaluation}) could then be solved as a set of LPs.

\begin{theorem}
    \label{theorem:BaB-correct}
    Algorithm \ref{algo:BaB} is sound and complete, i.e., $b(x)$ is positive invariant if and only if the algorithm returns $1$.
\end{theorem}

==> sections/Framework.tex <==
\section{Verification Framework}
\subsection{Enumerating Activation Sets}
Our approach to enumerating the activation sets that intersect with the safety boundary is as follows. Starting with an initial point $x$ with $b(x) = 0$ (which we compute by searching along a line between $x_{0}$ and $U_{i}$), we find an activation set $\mathbf{S} \in \mathbf{S}(x)$. We then identify all sets $\mathbf{S}^{\prime}$ such that there exists $x \in \overline{\mathcal{X}}(\mathbf{S}) \cap \overline{\mathcal{X}}(\mathbf{S}^{\prime})$ with $b(x) = 0$; we observe that such an $x$ can be computed by solving a linear program. We then find all sets $S^{\prime\prime}$ with $\overline{\mathcal{X}}(\mathbf{S}^{\prime}) \cap \overline{\mathcal{X}}(\mathbf{S}^{\prime\prime}) \cap \{x: b(x) = 0\} \neq \emptyset$, continuing until we have enumerated all such activation sets that are connected to $x$. This procedure is described in detail in Algorithms \ref{alg:Enumerate}.

\begin{algorithm}[h]
\caption{Enumerate Activated Sets}
\begin{algorithmic}[1]
    \State \textbf{Input:} State $x$ such that $b(x) = 0$
    \State \textbf{Output:} Set of activation sets $\mathcal{S}$ such that the connected component of the boundary containing $x$ is contained in $\bigcup_{\mathbf{S} \in \mathcal{S}}{\mathcal{X}(\mathbf{S})}$, set of activation sets with nonempty intersection $\mathcal{V}$
    \Procedure{Enumeration}{$x$}
    \State Uniformly sample $M$ points. The set $\mathcal{M}:=\{\Tilde{x}_i^{0}, i\in \{1,\ldots,M\}\}$ 
    \State Conduct gradient decent to identify points $\Tilde{x}_i$ such that $b(\Tilde{x}_i)\in (-\epsilon, \epsilon)$ for $i\in \{1,\ldots,M\}$. 
    \State Branch-and-Bound Search
    \State \textbf{Return} ActivationSetHelper($\mathbf{S}$, $\{\mathbf{S}\}$, $\{\mathbf{S}\}$)
   \EndProcedure
\end{algorithmic}
\label{alg:Enumerate}
\end{algorithm}

The following result describes the completeness guarantees of Algorithm \ref{alg:Enumerate}.

\begin{proposition}
\label{prop:enumeration-complete}
Let $\mathcal{S}$ and $\mathcal{V}$ denote the output of Algorithm \ref{alg:Enumerate}. Then the connected component of $\{x: b(x) = 0\}$ containing the input $x$, denoted $D$, satisfies $D \subseteq \bigcup_{\mathbf{S} \in \mathcal{S}}{\overline{\mathcal{X}}(\mathbf{S})}$. Furthermore, if $\mathbf{S}_{1},\ldots,\mathbf{S}_{r} \in \mathcal{S}$ is complete and $\left(\bigcap_{i=1}^{r}{\overline{\mathcal{X}}(\mathbf{S}_{i})}\right) \cap \{x: b(x) = 0\} \neq \emptyset$, then $\{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\} \in \mathcal{V}$.
\end{proposition}

\begin{proof}
Suppose that $x^{\prime} \in D \setminus \left(\bigcup_{\mathbf{S} \in \mathcal{S}}{\overline{\mathcal{X}}(\mathbf{S})}\right)$. Since $D$ is connected, there exists a path $\gamma$ with $\gamma(0) = x$ and $\gamma(1)=x^{\prime}$ contained in $D$. Let $\mathbf{S}_{0}, \mathbf{S}_{1},\ldots,S_{K}$ denote a sequence of activation patterns with $\mathbf{S}_{0} \in \mathbf{S}(x)$, $\mathbf{S}_{K} \in \mathbf{S}(x^{\prime})$, and $\mathbf{S}_{0}$ equal to the set computed at Line 3 of Algorithm \ref{alg:Enumerate}. Then there exists $i \geq 2$ such that $\mathbf{S}_{i-1} \in \mathcal{S}$ and $\mathbf{S}_{i} \notin \mathcal{S}$, and there exists $t^{\prime}$ such that $\gamma(t^{\prime}) \in \overline{\mathcal{X}}(\mathbf{S}_{i-1}) \cap \overline{\mathcal{X}}(\mathbf{S}_{i}) \cap \{x: b(x) = 0\}$. We then have that $\mathbf{T}(\mathbf{S}_{i-1},\mathbf{S}_{i})$ is a subset of the set $\mathbf{T}$ computed at Line 4 of Algorithm \ref{alg:EnumerateHelper}, and hence $\mathbf{S}_{i}$ will be identified and added to $\mathcal{S}$ at Line 7 of Algorithm \ref{alg:EnumerateHelper}. 

Now, suppose that $\mathbf{S}_{1},\ldots,\mathbf{S}_{r} \in \mathcal{S}$ is complete and $\left(\bigcap_{i=1}^{r}{\overline{\mathcal{X}}_{0}(\mathbf{S}_{i})}\right) \cap \{x: b(x) = 0\} \neq \emptyset$. Let $l$ denote the first index such that Algorithm \ref{alg:EnumerateHelper} is called with $\mathbf{S}_{l}$ as input; without loss of generality, suppose $l=1$. Let $\mathbf{T} = \mathbf{T}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r})$. Then $\mathbf{T}$ is a subset of of the set $T$ computed at line 4 of the algorithm, and the sets $\mathbf{S}_{1},\ldots,\mathbf{S}_{r}$ are enumerated at lines 7-13. Since the intersection of the $\overline{\mathcal{X}}(\mathbf{S})$ sets with $\{x: b(x) = 0\}$ is nonempty, $\{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\}$ is added to $\mathcal{V}$. 
\end{proof}

==> sections/Introduction/introV0.tex <==
\input{sections/timeline}
\section{Introduction}
\label{sec:intro}
% outline: 
% Safety of autonomous systems is important. 
% Deriving safety guarantee of NN-enabled system is challenging. 
% NCBF/NBC is current state of the art
% However, NCBFs synthesized by existing works may fail to ensure safety
% - better synthesis method to make NCBF verifiable safe is needed
% - Verification is needed for the generic ncbf training framework

% Existing verifiable synthesis encounters three challenges:
% 1. Existing CEGIS Cannot handle piece-wise linear NN (ReLU) very well
% 2. CE guided synthesis relies on verification. however existing verification suffers from curse of dimensionality. Poor scalability make them not scalable enough verification to be integrated into training efficiently

% In this paper, we propose synthesis with efficient exact verifiable synthesis (SEEV) for piece-wise linear NCBF. 
% SEEV is ...
% It addresses the first issue by adopting exact verification for piece-wise linear NCBFs
% It mitigates the curse of dimensionality in two major aspects. 
% 1. A universal way to represent piece-wise linear networks and an efficient verification that do not relies on the dimension of the system.  
% 2. A verification optimized synthesis to further boost verification by regularizing number activation sets to be verified. 

% Safety of autonomous systems is important. 
Safety, as a fundamental property, plays a significant role in medicine, energy, and robotics \cite{hsu2015control,agrawal2021safe} systems with applications involved with human lives and property security. The significance motivates a body of research into safety certificates [*ref] and safe control strategies \cite{xu2017correctness,breeden2021high, dai2023convex, kang2023verification,rober2023hybrid}. 
% BF provide safety guarantee
Barrier Functions (BFs) conceptualize the "barrier" of a dynamic system by identifying a set of states as the safe set, in which BFs remain non-negative. 
BF-based approaches show great promise in safety-critical systems by providing theoretical safety guarantees and flexibility to be integrated into various applications. 
These approaches can be roughly categorized into the Barrier Certificate (BC) and Control Barrier Functions (CBFs). 
The BC ensures the safety of dynamic systems by constructing a BF and certifies positive invariance property that any trajectory starting within the set with non-negative BF remains inside. 
The CBF provides a high degree of flexibility since any control policy that satisfies CBF constraints is safe and the system remains in the safe set for all time. 
% NCBF/NBC is current state of the art
Neural networks parameterized BFs (NBFs) have been proposed for BC [*ref] known as (Almost-BFs) and CBF-based safe control [*ref] known as (NCBF or NCLBF). NBFs show great promise in complex tasks due to the universal representability of neural networks and for high-dimensional dynamic systems due to efficient learning algorithms and better scalability compared to traditional Sum-Of-Square (SOS) based polynomial BF synthesis. 
% Deriving safety guarantee are invalidated by safety counterexamples 
However, recent research reveals the existence of safety counterexamples in both NBF-based BC [*ref] and NCBF-based safe control [*ref]. The safety counterexamples are states where the safety conditions do not hold invalidating the derived safety guarantees.
% However, NCBFs synthesized by existing works may fail to ensure safety. It is challenging
The synthesis of an NBF without safety counterexamples remains a challenging research problem. 

In this paper, we consider the problem of synthesizing verifiable-safe NBFs for continuous-time nonlinear control affine systems. Our focus is on NBFs represented by piece-wise linear feedforward neural networks for several compelling reasons. Firstly, networks such as ReLU NCBFs are extensively utilized in safe control research due to their robustness and efficacy. Secondly, piece-wise linear neural networks are favored for their promising representational capabilities [*ref nature hinge] and their rapid convergence during training [Appendix]. 
Given that NBFs are instrumental in deriving safety guarantees, it is crucial to ensure that these functions are verifiably safe, meaning they are devoid of any safety counterexamples.
The primary challenge in NBF synthesis lies in training networks that are both efficient and verifiably safe. This challenge emerges from two main factors: the need for safety verification and the demand for efficient synthesis. On one hand, verifying neural networks remains a largely unresolved issue in the research community. Most existing verification methodologies struggle with the curse of dimensionality, which significantly hampers scalability as system dimensions increase. On the other hand, there is an inherent contradiction between efficient training and thorough safety verification, as the latter requires substantial computational resources.
% The key challenge of NBFs synthesis is to efficiently train verifiable safe NBFs. The challenge comes from two factors, safety verification and efficient synthesis. On one hand, the verification of neural networks is an open research problem. Most existing verification methodologies suffer from the curse of dimensionality, i.e., they do not scale well as the dimension increases. On the other hand, efficient training fundamentally contradicts safety verification since it takes extra computational resources. 


% Existing verifiable synthesis encounters two challenges:
% 1. efficient synthesis may result in CE
\textcolor{blue}{[CE] from existing works
Almost-Barrier Function [Zhizhen IROS] propose an efficient algorithm to synthesize NBFs with almost sure guarantees. [Can we have a motivating example here?]}
% 2. Existing CEGIS Cannot handle piece-wise linear NN (ReLU) very well. CE guided synthesis relies on verification.
Counterexample-guided synthesis (CEGIS), crucially dependent on reliable verification, encounters difficulties with piece-wise linear neural networks, such as those employing ReLU activation functions. Specifically, SMT-based verifiers, which are commonly used in CEGIS, do not scale well. This scaling issue hinders their effective integration into the training process, severely limiting the applicability of CEGIS to these neural networks.
% 2. existing verification suffers from curse of dimensionality. Poor scalability make them not scalable enough verification to be integrated into training efficiently
% Exact verification of ReLU NCBFs is proposed to provide theoretical guarantees. It adopts sampling based neural network approximation technique to overapproximate the boundary of NBFs. However, its approximation technique suffers from the curse of dimensionality. Poor scalability makes it not scalable enough to be integrated into the synthesis framework. 
Furthermore, the exact verification of ReLU NCBFs, while offering theoretical safety guarantees, adopts a sampling-based neural network approximation technique to overapproximate the boundaries of NBFs. Unfortunately, this method is also plagued by the curse of dimensionality. 
% - better synthesis method to make NCBF verifiable safe is needed
% - Verification is needed for the generic ncbf training framework
The evident gap in the verifiable synthesis of piece-wise linear Neural-network parameterized Barrier Functions (NBFs) highlights a crucial demand for innovative approaches. These approaches must be capable of managing the complexity and dimensional challenges inherent in these systems, emphasizing the need for advanced solutions that can effectively navigate the intricacies of piece-wise linear neural networks.

% In this paper, we propose synthesis with efficient exact verification (SEEV) for piece-wise linear NCBF. SEEV consists of a regulator to guide training a verifiable safe NBF and easy to verify, a regulator and counterexample guided synthesis framework and an efficient exact verifier to provide safety guarantee if pass and safety counterexample for retraining. 
In this paper, we introduce the Synthesis with Efficient Exact Verification (SEEV) approach for piece-wise linear Neural Control Barrier Functions (NCBF). SEEV integrates a regulator to guide the training of a verifiably safe NBF, which is also straightforward to verify, alongside a counterexample-guided synthesis framework and an efficient exact verifier. This verifier not only provides safety guarantees upon successful verification but also generates safety counterexamples for subsequent retraining.
% It mitigates the curse of dimensionality in two major aspects. 
% We utilize a universal way to represent piece-wise linear networks and an efficient verification that do not relies on the dimension of the system. Activation of each neuron allows us to fully utilize the piece-wise linear characteristic of ReLU network and represent the network with linear expression in a certain small domain. Naguno's theorem allows us to conduct exact verification by verifying all the boundary linear segments. Based on these characteristics, an efficient verifier is proposed to perform linear programs for searching and nonlinear programs for verification. 
SEEV mitigates the curse of dimensionality in two primary ways. First, we adopt a universal representation for piece-wise linear networks that does not rely on system dimensionality. This is achieved by activating each neuron to fully utilize the piece-wise linear nature of ReLU networks, representing the network with linear expressions within defined small domains. Furthermore, leveraging Nagumo's theorem, we conduct exact verifications by scrutinizing all boundary linear segments. the regulators are designed to penalize potential safety risks and regulate the number of boundary linear segments. Second, based on our observation shown in [appendix], the scalability of the verification problem majorly relies on the number of boundary segments and the number of total neurons. we adopt a regulator to cut down the number of boundary linear segments. 
% To address the efficiency issue, we improve the efficiency of both verifier and trainer. The verifier is designed to work parallelly and output safety counterexamples for retraining. The regulators are designed to penalize potential safety counterexamples and regularize the number boundary linear segments. The synthesis framework balance between regulators and counterexamples for efficiency.
To enhance efficiency, our approach improves both the verifier and the trainer. The verifier operates in parallel, providing safety counterexamples that feed into the retraining process. Meanwhile, the regulators are designed to penalize potential safety risks and regulate the number of boundary linear segments. This synthesis framework carefully balances regulators and counterexamples to optimize efficiency, ensuring a robust process that enhances the verifiability and safety of piece-wise linear NCBFs.



==> sections/Introduction/introV1.tex <==
\section{Introduction}
\label{sec:intro}

% Safety of autonomous systems is important. 
Safety, as an essential attribute, is crucial in domains such as medicine, energy, and robotics, where human lives and property are at risk \cite{hsu2015control,agrawal2021safe}. This criticality has spurred extensive research into safety certificates [*ref] and advanced safe control strategies \cite{xu2017correctness,breeden2021high, dai2023convex, kang2023verification,rober2023hybrid}.
% BF provide safety guarantee
Control Barrier Functions (BFs) are fundamental in conceptualizing the "barrier" of a dynamic system, defining a set of states known as the safe set, wherein the CBFs remain non-negative. CBF-based methodologies offer significant theoretical safety guarantees and versatility, allowing for integration across various applications. These methodologies are primarily divided into Barrier Certificates (BCs) and Control Barrier Functions (CBFs). BCs ensure the safety of dynamic systems by constructing a CBF that certifies the positive invariance property of a feedback-controlled system, ensuring that any trajectory starting within the safe set remains contained. CBFs provide considerable flexibility, ensuring that any control policy meeting CBF criteria maintains system safety over time.
% NCBF/NBC is current state of the art
Recently, Neural-network parameterized CBFs (NCBFs) have been introduced for BCs, referred to as Almost-BFs, and for CBF-based safe control, known as NCBFs or NCLBFs [*ref]. NBFs are particularly promising for complex tasks due to the universal representability of neural networks and their superior scalability and efficiency in learning algorithms compared to traditional Sum-Of-Squares (SOS) based polynomial BF synthesis.
% Deriving safety guarantee are invalidated by safety counterexamples 
However, recent studies have identified safety counterexamples in NCBFs. These counterexamples are specific states where the safety conditions fail, thereby invalidating the derived safety guarantees. 
% However, NCBFs synthesized by existing works may fail to ensure safety. It is challenging
% The synthesis of an NBF without safety counterexamples remains a challenging research problem. 
Consequently, developing an NCBF that reliably avoids safety counterexamples presents a significant and ongoing challenge in the field.

In this paper, we consider the problem of synthesizing verifiable-safe NCBFs for continuous-time nonlinear control affine systems. Our focus is on NCBFs represented by piece-wise linear feedforward neural networks for several compelling reasons. Firstly, networks such as ReLU NCBFs are extensively utilized in safe control research due to their robustness and efficacy. Secondly, piece-wise linear neural networks are favored for their promising representational capabilities [*ref nature hinge] and their rapid convergence during training [Appendix]. 
Given that NCBFs are instrumental in deriving safety guarantees, it is crucial to ensure that these functions are verifiably safe, meaning they are devoid of any safety counterexamples.
The primary challenge in NCBF synthesis lies in training networks that are both efficient and verifiably safe. This challenge emerges from two main factors: the need for safety verification and the demand for efficient synthesis. On one hand, verifying neural networks remains a largely unresolved issue in the research community. Most existing verification methodologies struggle with the curse of dimensionality, which significantly hampers scalability as system dimensions increase. On the other hand, there is an inherent contradiction between efficient training and thorough safety verification, as the latter requires substantial computational resources.
% The key challenge of NBFs synthesis is to efficiently train verifiable safe NBFs. The challenge comes from two factors, safety verification and efficient synthesis. On one hand, the verification of neural networks is an open research problem. Most existing verification methodologies suffer from the curse of dimensionality, i.e., they do not scale well as the dimension increases. On the other hand, efficient training fundamentally contradicts safety verification since it takes extra computational resources. 


% Existing verifiable synthesis encounters two challenges:
% 1. efficient synthesis may result in CE
\textcolor{blue}{[Zhizhen: Done.] In practice, synthesizing verifiable NCBFs from samples is often challenging, and counterexamples from verifications frequently need to be added to the training dataset to enhance verifiability [cite Zhizhen IROS]. This adversarial training loop is commonly known as Counterexample-Guided Inductive Synthesis (CEGIS). }
%[CE] from existing works. Almost-Barrier Function [Zhizhen IROS] propose an efficient algorithm to synthesize NCBFs with almost sure guarantees. [Can we have a motivating example here?]}
% 2. Existing CEGIS Cannot handle piece-wise linear NN (ReLU) very well. CE guided synthesis relies on verification.
CEGIS, crucially dependent on reliable verification, encounters difficulties with piece-wise linear neural networks, such as those employing ReLU activation functions. Specifically, SMT-based verifiers, which are commonly used in CEGIS, do not scale well. This scaling issue hinders their effective integration into the training process, severely limiting the applicability of CEGIS to these neural networks.
% 2. existing verification suffers from curse of dimensionality. Poor scalability make them not scalable enough verification to be integrated into training efficiently
% Exact verification of ReLU NCBFs is proposed to provide theoretical guarantees. It adopts sampling based neural network approximation technique to overapproximate the boundary of NBFs. However, its approximation technique suffers from the curse of dimensionality. Poor scalability makes it not scalable enough to be integrated into the synthesis framework. 
Furthermore, the exact verification of ReLU NCBFs, while offering theoretical safety guarantees, adopts a sampling-based neural network approximation technique to overapproximate the boundaries of NBFs. Unfortunately, this method is also plagued by the curse of dimensionality. 
% - better synthesis method to make NCBF verifiable safe is needed
% - Verification is needed for the generic ncbf training framework
The evident gap in the verifiable synthesis of piece-wise linear Neural-network parameterized NCBFs highlights a crucial demand for innovative approaches. These approaches must be capable of managing the complexity and dimensional challenges inherent in these systems, emphasizing the need for advanced solutions that can effectively navigate the intricacies of piece-wise linear neural networks.

% In this paper, we propose synthesis with efficient exact verification (SEEV) for piece-wise linear NCBF. SEEV consists of a regulator to guide training a verifiable safe NBF and easy to verify, a regulator and counterexample guided synthesis framework and an efficient exact verifier to provide safety guarantee if pass and safety counterexample for retraining. 
In this paper, we introduce the Synthesis with Efficient Exact Verification (SEEV) approach for piece-wise linear Neural Control Barrier Functions (NCBF). SEEV integrates a regulator to guide the training of a verifiably safe NCBF, which is also straightforward to verify, alongside a counterexample-guided synthesis framework and an efficient exact verifier. This verifier not only provides safety guarantees upon successful verification but also generates safety counterexamples for subsequent retraining.
% SEEV mitigates the curse of dimensionality in two primary ways. First, we adopt a universal representation for piece-wise linear networks that does not rely on system dimensionality. This is achieved by activating each neuron to fully utilize the piece-wise linear nature of ReLU networks, representing the network with linear expressions within defined small domains. Furthermore, leveraging Nagumo's theorem, we conduct exact verifications by scrutinizing all boundary linear segments. the regulators are designed to penalize potential safety risks and regulate the number of boundary linear segments. Second, based on our observation shown in [appendix], the scalability of the verification problem majorly relies on the number of boundary segments and the number of total neurons. we adopt a regulator to cut down the number of boundary linear segments. 
SEEV effectively mitigates the curse of dimensionality through two primary strategies. First, it adopts a universal representation for piece-wise linear networks that does not depend on system dimensionality. This is facilitated by activating each neuron to capitalize on the piece-wise linear characteristics of ReLU networks, allowing the network to be represented by linear expressions within specifically defined small domains. Moreover, by leveraging Nagumo's theorem, SEEV conducts exact verifications by meticulously scrutinizing all boundary linear segments.
Secondly, as indicated in our findings detailed in the [appendix], the scalability of the verification problem is principally influenced by the number of boundary segments and the total number of neurons. In response, SEEV incorporates a regulator specifically designed to reduce the number of boundary linear segments, thereby streamlining the verification process.
% To enhance efficiency, our approach improves both the verifier and the trainer. The verifier operates in parallel, providing safety counterexamples that feed into the retraining process. Meanwhile, the regulators are designed to penalize potential safety risks and regulate the number of boundary linear segments. This synthesis framework carefully balances regulators and counterexamples to optimize efficiency, ensuring a robust process that enhances the verifiability and safety of piece-wise linear NCBFs.
To boost overall efficiency, SEEV enhances both the verifier and the trainer. The verifier operates in parallel, efficiently producing safety counterexamples that are integral to the retraining process. Additionally, the regulators are strategically designed to not only penalize potential safety risks but also to control the number of boundary linear segments. This synthesis framework skillfully balances the roles of regulators and counterexamples to optimize efficiency, thus ensuring a robust process that significantly enhances the verifiability and safety of piece-wise linear NCBFs.

\input{sections/Introduction/relatedV0}

\input{sections/Introduction/organization}

==> sections/Introduction/relatedV0.tex <==
\textbf{Related Work}

!Synthesis
Neural barrier certificate~\cite{berkenkamp2017safe,abate2021fossil,qin2021learning,qin2022quantifying} and NCBFs~\cite{dawson2022safe,dawson2023safe,liu2023safe} have been proposed to describe complex safety constraints that cannot be encoded polynomials. 

!Verification
mixed-integer programs \cite{zhao2022verifying}, and 

Sum-of-squares (SOS) optimization and other techniques derived from algebraic geometry have been widely used for safety verification of polynomial barrier functions \cite{prajna2007framework,ames2019control,zhao2022safety,schneeberger2023sos,clark2021verification}. 
% However,  SOS-based approaches cannot be directly applied to NCBF verification, since activation functions used in neural networks are not polynomial and can be non-differentiable.
However, SOS-based approaches for polynomial CBFs cannot be applied directly to NCBF verification, since activation functions used in neural networks are not polynomial and may be non-differentiable.


verify input/output relationships \cite{ferrari2022complete,henriksen2021deepsplit,zhang2022general} and ReLU neural networks focused verification~\cite{katz2017reluplex,katz2019marabou}. These methods, however, are not directly applicable to the problem of NCBF verification

nonlinear programs \cite{zhang2023exact}


Solely introducing verifiers into the training loop to filter out the ones who failed the verification may not result in training a verifiable result. 


!Synthesis with verifiable guarantees. 
Counterexample Guided 
SMT-based techniques \cite{zhao2020synthesizing,abate2021fossil,abate2020formal,10.1007/978-3-030-72016-2_20}, 
\cite{anand2023formally}

However, SMT-based approach does not scale well with the network size increases. 
sampling-based approach may \cite{anand2023formally,tayal2024learning} prove safety by Lipschitz condition relies on the assumption of Lipschitz on NCBF and do not scale well due to the assumption on dense sampling over the state space. 

whereas in this work we present a 

% Existing verifiable training either
% Training schemes based on this training dataset usually assume a dense sampling \cite{anand2023formally,tayal2024learning} and prove safety by Lipschitz condition. The key idea of the assumption is to collect training data on the boundary to train and prove safety by Lipschitz condition. However, approaches based on the assumption do not scale well in high-dimensional cases.

% including learning from expert demonstrations \cite{9303785}, SMT-based techniques \cite{zhao2020synthesizing,abate2021fossil,abate2020formal,10.1007/978-3-030-72016-2_20}, mixed-integer programs \cite{zhao2022verifying}, and nonlinear programs \cite{zhang}. Loss functions for training NCBFs were proposed in \cite{dawson2022safe,dawson2023safe,liu2023safe,9993334,zhang2024fault}, while  \cite{so2023train} synthesizes CBFs by learning a value function of a nominal policy and demonstrating that the maximum-over-time cost serves as a CBF.
Neural barrier certificates~\cite{berkenkamp2017safe,abate2021fossil,qin2021learning,qin2022quantifying} and Neural Control Barrier Functions (NCBFs)~\cite{dawson2022safe,dawson2023safe,liu2023safe} have been proposed to describe complex safety constraints that cannot be encoded as polynomials. These methods leverage the expressiveness of neural networks to ensure safety in nonlinear systems. For instance, Berkenkamp et al.~\cite{berkenkamp2017safe} introduced techniques for safe learning in control using Gaussian processes, while Abate et al.~\cite{abate2021fossil} developed Fossil, a tool for the formal synthesis of Lyapunov functions and barrier certificates using neural networks. Qin et al.~\cite{qin2021learning, qin2022quantifying} focused on learning and quantifying safety for systems where polynomial methods fall short. Dawson et al.~\cite{dawson2022safe, dawson2023safe} and Liu et al.~\cite{liu2023safe} further demonstrated the application of NCBFs in various complex systems.

\subsection{Verification}
Verification of safety properties in neural networks has utilized several approaches. Mixed-integer programs (MIP)~\cite{zhao2022verifying} offer one method, though they face significant computational challenges. Sum-of-squares (SOS) optimization~\cite{prajna2007framework, ames2019control, zhao2022safety, schneeberger2023sos, clark2021verification} has been widely used for polynomial barrier functions, but these methods are not applicable to NCBFs due to the non-polynomial and potentially non-differentiable activation functions in neural networks. Methods for verifying input/output relationships~\cite{ferrari2022complete, henriksen2021deepsplit, zhang2022general} and ReLU neural networks~\cite{katz2017reluplex, katz2019marabou} are also not directly applicable to NCBF verification. Nonlinear programming approaches~\cite{zhang2023exact} provide another route for exact verification but are computationally intensive.

\subsection{Synthesis with Verifiable Guarantees}
To synthesize neural networks with verifiable guarantees, Counterexample Guided Inductive Synthesis (CEGIS) has been applied using SMT-based techniques~\cite{zhao2020synthesizing, abate2021fossil, abate2020formal, 10.1007/978-3-030-72016-2_20, anand2023formally}. However, SMT-based methods do not scale well with increasing network size. Sampling-based approaches~\cite{anand2023formally, tayal2024learning} aim to prove safety using Lipschitz conditions, but they rely on dense sampling over the state space, which is computationally prohibitive.

\subsection{Current Work}
In this work, we present a framework for Synthesis with Efficient Exact Verification (SEEV) for NCBFs. Our method addresses the computational bottlenecks of existing techniques by introducing a regularizer to reduce the number of activation regions and leveraging efficient enumeration algorithms. By integrating synthesis and verification components within the training loop, we ensure verifiable safety guarantees for high-dimensional systems.


==> sections/Synthesis/LossDesignV0.tex <==
\subsection{Loss Function Design}
\label{subsec:lossdesign}
% Loss Design
    % Observation pointing out the bottleneck is equivalent to regularizing the number of boundary hyperplanes
    % Regulator design: 1. correctness regulator. 2. feasibility loss. 3. number of boundary hyperplanes
    % Loss function: sum of weighted losses. The idea behind design. 
    % Priority Design: adaptive weight allocation based on CE type. logic and numerical support Priority-based Efficiency optimize

Let $\theta$ denote all trainable weight $\mathbf{W}$ and bias $\mathbf{r}$ of the NCBF. We denote the entity determined by parameter $\theta$ using subscript, i.e., the safety set $\mathcal{D}_{\theta}$ and linear hyperplanes $\overline{\mathcal{X}}_{\theta}$.  
\sysname aims to synthesize valid NCBFs without safety counterexamples and is easy to verify. To synthesize valid NCBFs without safety counterexamples, the Problem \ref{prob:synth} is to optimize $\theta$ such that (i) \eqref{eq:neural-containment} holds; (ii) \eqref{eq:safety-condition-1}-\eqref{eq:safety-condition-2} hold for all $x\in \partial \mathcal{D}_{\theta}$. Let set $\mathcal{B}_{\theta}:=\{\mathbf{S}_i: \partial\mathcal{D}_{\theta} \cap \overline{\mathcal{X}}_{\theta}(\mathbf{S}_i)\neq \emptyset\}$ denote the activation set that contains safety boundary $\partial\mathcal{D}$. 
As shown in Appendix \ref{appendix:sssec:regularizer}, the synthesized NCBF is easier to verify as the number of boundary hyperplanes decreases, i.e., the cardinality of set $\|\mathcal{B}\|$ decreases. The optimization program is given as follows. 
\begin{align}
    \label{eq:train_obj}
    \min_{\theta}&\quad{\|\mathcal{B}_{\theta}\|} \\
    s.t. &\quad \eqref{eq:safety-condition-1}-\eqref{eq:safety-condition-2}, \quad \forall x\in \partial\mathcal{D}_{\theta} \\
    &\quad \eqref{eq:neural-containment}, \mathcal{I} \subseteq \mathcal{D}_{\theta}
\end{align}
However, it is challenging to train by solving the constrained optimization problem. In this work, we convert the constrained optimization to an unconstrained one by constructing a loss function that penalizes violations of the constraints. We enforce the constraints by employing the verifier and we formulate the following unconstrained optimization problem to search for $\theta$. 
\begin{equation}
    \label{eq:uncons_opt}
    \min_{\theta}\quad{\lambda_\mathcal{B}\mathcal{L}_\mathcal{B}(\mathcal{T})} + \lambda_{f}\mathcal{L}_f(\mathcal{T}) + \lambda_{c}\mathcal{L}_c(\mathcal{T}) 
\end{equation}
where $\mathcal{L}_\mathcal{B}(\mathcal{T})$ approximate $\|\mathcal{B}_{\theta}\|$, $\mathcal{L}_f(\mathcal{T})$ is the loss penalizing the violations of constraint \eqref{eq:safety-condition-1}-\eqref{eq:safety-condition-2}, $\mathcal{L}_c(\mathcal{T})$ penalizes the violations of constraint \eqref{eq:neural-containment}, and $\lambda_\mathcal{B}$, $\lambda_{f}$ and $\lambda_{c}$ are non-negative coefficients. The detailed design of $\mathcal{L}_f$, $\mathcal{L}_c$ are in [appendix]. 
In what follows, we detail the regularizer for $\mathcal{L}_\mathcal{B}$. 

\textbf{$\mathcal{L}_\mathcal{B}$ Regularizer:} We propose a novel regularization technique aimed at encouraging similar activation patterns for samples located along the safety boundary, denoted as \( \mathcal{X}_{bs} \). For each individual sample \( x \in \mathcal{X}_{bs}\), we extract its activation pattern by concatenating the activation patterns from each post-ReLU layer. We designed a loss function that minimizes the distance between the activation patterns of samples within \( \mathcal{X}_{bs} \). This loss function is expressed as:

\[
\mathcal{L}_{\text{reg}} = \frac{1}{|\mathcal{X}_{bs}|^2} \sum_{i, j \in \mathcal{X}_{bs}} \| \phi(x_i) - \phi(x_j) \|_2^2,
\]

where \( \phi(x) \) represents the concatenated activation pattern of sample \( x \).

Two techniques are necessary to effectively apply this regularizer in practice. First, to ensure that the activation pattern extraction process is differentiable, we use a modified sigmoid function, \( \sigma_k(p) = \frac{1}{1 + \exp(-k \cdot p)} \), on each pre-activated feature \( p \). By choosing a sufficiently large \( k \), this modified sigmoid function approximates the behavior of the sign function while maintaining gradient information. We denote the approximated activation pattern of input \( x \) as \( \phi_{\sigma_k}(x) \).

Second, rather than applying the regularization across the entire set \( \mathcal{X}_{bs} \), we employ unsupervised learning to group the samples into clusters. The regularizer is then applied within each cluster. This approach ensures that we only encourage similar activation patterns within reasonable neighborhoods, thereby avoiding the potential pitfalls of enforcing similarity across the entire boundary set.

The final regularization loss can be expressed as:

\[
\mathcal{L}_{\mathcal{B}} = \frac{1}{|\mathcal{C}|} \sum_{c \in \mathcal{C}} \frac{1}{|c|^2} \sum_{i, j \in c} \| \phi_{\sigma_k}(x_i) - \phi_{\sigma_k}(x_j) \|_2^2,
\]

where the inner sum iterates over all pairs of samples within each cluster \( c \).


==> sections/Synthesis/OverviewV0.tex <==
\subsection{Overview}
\label{subsec:synth_overview}

% Overview
    % Problem Formulation
    % challenges: 1. no guarantee. 2. low efficiency. 3. converge slow
    % components to address challenges. 1. verifier embedded training. 2. efficient verification and regulator to speed verification. 3. exact counterexamples with designated guidance based on CE type. 
    % overall pipeline and high-level description 
    % regulator for getting close to satisfying the condition in verification (lie derivative)
    % regulator to limit the segments 
    
% Ensure that the synthesized $ b_{\theta}(x) $ adheres to the rigorous safety conditions derived from adaptations of Nagumo's theorem, suitable for nonsmooth boundaries.
% Manage the computational scalability challenges that arise as neural network size and dimensionality increase.

We consider the scenario where the system \eqref{eq:dynamics} must remain within a designated safety set $\mathcal{C}$. Our primary objective is to synthesize a ReLU Neural Control Barrier Function (ReLU-NCBF) for the dynamic system and subsequently develop a safe control policy to ensure system safety.

\begin{problem}
\label{prob:synth}
    Given a system \eqref{eq:dynamics} and a safety set $\mathcal{C}$, synthesize a ReLU NCBF $b_{\theta}(x)$ parameterized by $\theta$ such that the conditions in Proposition \ref{prop:safety-condition} are satisfied. Then construct a control policy to synthesize $u_{t}$ such that the system remains positive invariant in set $\mathcal{D}:=\{x: b(x)\geq0\}\subseteq \mathcal{C}$. 
\end{problem}

Addressing Problem \ref{prob:synth} presents several challenges: 
(i) Synthesizing an NCBF that is guaranteed to be counterexample-free is non-trivial.
(ii) The integration of verifiers into the training framework leads to a significant efficiency drop due to the scalability issues of NCBF verifiers.
(iii) Counterexample-guided training may not effectively guide the training process towards convergence. Safety counterexamples can fail to meet various conditions in Proposition \ref{prop:safety-condition}, and there is currently no systematic approach to categorize these counterexamples and provide appropriate treatments.

% components to address challenges. 1. verifier embedded training. 2. efficient verification and regulator to speed verification. 3. exact counterexamples with designated guidance based on CE type. 
% overall pipeline and high-level description 
% regulator for getting close to satisfying the condition in verification (lie derivative)
% regulator to limit the segments 
In this section, we propose \sysname to address the challenges. \sysname is a training framework designed to synthesize ReLU NCBF without safety counterexamples. The figure illustrates the \sysname framework. 
The NCBF training consists of three key regularizers: correctness, feasibility, and boundary activation. The correctness regularizer ensures adherence to safety conditions, the feasibility regularizer ensures the correct Lie derivative, and the boundary activation regulator limits the number of hyperplanes and hinges to manage scalability. 
During training, the boundary of the NCBF is identified by the Boundary Identification module and subsequently verified by the exact verifier. If the NCBF passes verification, it is deemed a Verified NCBF; if not, counterexamples are fed back into the training process for iterative improvement. 
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figs/trainingframework.jpg}
    \caption{\sysname: Synthesis with Efficient Exact Verifier for ReLU NCBF}
    \label{fig:synthframe}
\end{figure}

% In this section, we propose \sysname to address the challenges. \sysname is a training framework for ReLU NCBF. The framework consists of an verifier, regularizer and counterexample guided training. \sysname adopts an efficient exact verifier to ensure the synthesized $b_{\theta}(x)$ meets the rigorous safety conditions in Proposition \ref{prop:safety-condition} to address the first challenge. The verifier utilize the piecewise linear characteristic of the ReLU NCBF, decompose the verification problem into linear and nonlinear programming problems and efficiently certify or identify safety counterexamples. The benefit of an efficient verifier mitigate the scalability issue in the second challenge. 
To address the first challenge, \sysname employs an efficient exact verifier to ensure that the synthesized $b_{\theta}(x)$ meets the rigorous safety conditions outlined in Proposition \ref{prop:safety-condition}. The verifier leverages the piecewise linear nature of the ReLU NCBF and decomposes the verification problem into linear and nonlinear programming tasks. This method efficiently certifies safety or identifies counterexamples, thereby mitigating the scalability issues highlighted in the second challenge.
% \sysname leverages a set of regularizers to guide the NCBF to satisfy conditions in Proposition \ref{prop:safety-condition} and to improve the efficiency of verification. Our observation [appendix] shows that the runtime of the verifier is majorly determined by the number of hyperplanes and hinges. The regularizer effectively limits the number of boundary hyperplanes and hinges to manage computational scalability challenges as neural network size and dimensionality increase.
\sysname also uses a set of regularizers to guide the NCBF in satisfying the conditions of Proposition \ref{prop:safety-condition} and to enhance verification efficiency. As our observations in the appendix indicate, the verifier's runtime is primarily influenced by the number of hyperplanes and hinges. The regularizers effectively limit the number of boundary hyperplanes and hinges, addressing the computational scalability challenges that arise as neural network size and dimensionality increase.
% \sysname balancing the roles of regularizers and counterexamples by utilizing a set of coarser to finer guide during training and a counterexample-guided training with categorical profiling. 
Furthermore, \sysname balances the roles of regularizers and counterexamples by implementing a multi-tiered guidance system during training, moving from coarser to finer granularity. This approach, combined with counterexample-guided training that includes categorical profiling, ensures targeted and effective improvements throughout the training process and hence mitigate the third challenge.


==> sections/Synthesis/OverviewV1.tex <==
\subsection{Overview}
\label{subsec:synth_overview}

% Overview
    % Problem Formulation
    % challenges: 1. no guarantee. 2. low efficiency. 3. converge slow
    % components to address challenges. 1. verifier embedded training. 2. efficient verification and regulator to speed verification. 3. exact counterexamples with designated guidance based on CE type. 
    % overall pipeline and high-level description 
    % regulator for getting close to satisfying the condition in verification (lie derivative)
    % regulator to limit the segments 
    
% Have the same initial paragraph and Problem 1.
% We consider the scenario where the system \eqref{eq:dynamics}, initialized within a given set $\mathcal{I}$, must remain within a designated safety set $\mathcal{C}$ and avoid $\mathcal{X}\backslash \mathcal{C}$. 
Our primary objective is to synthesize a ReLU Neural Control Barrier Function (ReLU-NCBF) for the dynamic system and subsequently develop a safe control policy to ensure system safety.

\begin{problem}
\label{prob:synth}
    Given a system \eqref{eq:dynamics}, initial set $\mathcal{I}$ and a safety set $\mathcal{C}$, synthesize a ReLU NCBF $b_{\theta}(x)$ parameterized by $\theta$ such that the conditions in Proposition \ref{prop:safety-condition} are satisfied. Then construct a control policy to synthesize $u_{t}$ such that the system remains positive invariant in set $\mathcal{D}:=\{x: b_{\theta}(x)\geq0\}$ and $\mathcal{I} \subseteq \mathcal{D} \subseteq \mathcal{C}$. 
\end{problem}

The inner loop attempts to choose parameter $\theta$ of the NCBF to satisfy the safety condition by minimizing the loss function over a training dataset we generated. 
The outer loop validates a given NCBF $b_\theta(x)$ by checking for safety counterexamples and updates the training dataset. 

% We propose \sysname to address this problem with the synthesis framework demonstrated in Fig. \ref{fig:synthframe}. The training framework consists of two loops. The outer loop validates a given NCBF $b_\theta(x)$ by checking for safety counterexamples and updates the training dataset. The inner loop attempts to guide the NCBF to satisfy the safety condition by minimizing the loss function. 

% There is an outer loop that takes a given NCBF b_\theta, checks for counterexamples, and updates the training dataset. The inner loop attempts to find an NCBF that minimizes the loss function.
% Say that in order to choose the parameters of the neural CBF in order to satisfy the conditions of Proposition 1, we propose a loss function that penalizes the NCBF for violating constraints (i) and (ii) at a collection of sample points.

To train the parameters of the NCBF satisfying the conditions of Proposition \ref{prop:safety-condition}, we propose a loss function that penalizes the NCBF for violating constraints (i) and (ii) at a collection of sample points. The loss function is a weighted sum of three terms. \textcolor{blue}{the first term is .. the second ... } The correctness loss ensures adherence to safety conditions and ensures that there exists a control input satisfying \eqref{eq:safety-condition-1}-\eqref{eq:safety-condition-2}. 
\textcolor{blue}{Minimizing the loss function is insufficient to ensure safety because there may exist safety counterexamples outside of the training dataset.} 
However, the safety may not be guaranteed solely by losses converging to zero \cite{so2023train}. The conditions hold for all training data may not necessarily mean they hold for all states since the training dataset is a subset of the state space. It is non-trivial for this approach to produce an NCBF that is guaranteed to be counterexample-free. In order to ensure safety, \sysname employs an efficient exact verifier to ensure that the synthesized $b_{\theta}(x)$ meets the safety conditions outlined in Proposition \ref{prop:safety-condition}. The verifier either produces a proof of safety, or generates a safety counterexample that can be added to the training dataset to improve the NCBF. 
% Then say that, while this approach can lead to provable safety, the safety verifier introduces significant additional computation.

\textcolor{blue}{improve safety}
Although this approach can lead to provable safety guarantees, the integration of the verifier leads to a significant additional computation.
% We mitigate this computation in two ways. Then you talk about the regularizer to reduce the number of activation patterns at the boundary. Second, you talk about the multi-tiered guidance system. 
We mitigate this computation in two ways. First \sysname employs an efficient verifier that mitigates the computational scalability challenges that arise as neural network depth and dimensionality increase. Second, \sysname adopts the regularizers to limit the number of boundary hyperplanes and hinges to be verified, addressing the computational scalability challenges that arise as neural network size increases.
\textcolor{blue}{First, we propose ... in section 4 that mitigate the scalability issue by .. . Second we introduces a regularizer}
% Furthermore, \sysname balances the roles of regularizers and counterexamples by implementing a multi-tiered guidance system during training, moving from coarser to finer granularity. This approach, combined with counterexample-guided training that includes categorical profiling, ensures targeted and effective improvements throughout the training process.

% Addressing Problem \ref{prob:synth} presents several challenges: 
% (i) Synthesizing an NCBF that is guaranteed to be counterexample-free is non-trivial.
% (ii) The integration of verifiers into the training framework leads to a significant efficiency drop due to the scalability issues of NCBF verifiers.
% (iii) Counterexample-guided training may not effectively guide the training process towards convergence. Safety counterexamples can fail to meet various conditions in Proposition \ref{prop:safety-condition}, and there is currently no systematic approach to categorize these counterexamples and provide appropriate treatments.

% components to address challenges. 1. verifier embedded training. 2. efficient verification and regulator to speed verification. 3. exact counterexamples with designated guidance based on CE type. 
% overall pipeline and high-level description 
% regulator for getting close to satisfying the condition in verification (lie derivative)
% regulator to limit the segments 

% In this section, we propose \sysname to address the challenges. \sysname is a training framework designed to synthesize ReLU NCBF without safety counterexamples. The figure illustrates the \sysname framework. 
% The NCBF training consists of three key regularizers: correctness, feasibility, and boundary activation. The correctness regularizer ensures adherence to safety conditions, the feasibility regularizer ensures the correct Lie derivative and the boundary activation regulator limits the number of hyperplanes and hinges to manage scalability. 
% During training, the boundary of the NCBF is identified by the Boundary Identification module and subsequently verified by the exact verifier. If the NCBF passes verification, it is deemed a Verified NCBF; if not, counterexamples are fed back into the training process for iterative improvement. 
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figs/trainingframework.jpg}
    \caption{\sysname: Synthesis with Efficient Exact Verifier for ReLU NCBF}
    \label{fig:synthframe}
\end{figure}

% In this section, we propose \sysname to address the challenges. \sysname is a training framework for ReLU NCBF. The framework consists of an verifier, regularizer and counterexample guided training. \sysname adopts an efficient exact verifier to ensure the synthesized $b_{\theta}(x)$ meets the rigorous safety conditions in Proposition \ref{prop:safety-condition} to address the first challenge. The verifier utilize the piecewise linear characteristic of the ReLU NCBF, decompose the verification problem into linear and nonlinear programming problems and efficiently certify or identify safety counterexamples. The benefit of an efficient verifier mitigate the scalability issue in the second challenge. 
% To address the first challenge, \sysname employs an efficient exact verifier to ensure that the synthesized $b_{\theta}(x)$ meets the rigorous safety conditions outlined in Proposition \ref{prop:safety-condition}. The verifier leverages the piecewise linear nature of the ReLU NCBF and decomposes the verification problem into linear and nonlinear programming tasks. This method efficiently certifies safety or identifies counterexamples, thereby mitigating the scalability issues highlighted in the second challenge.
% \sysname leverages a set of regularizers to guide the NCBF to satisfy conditions in Proposition \ref{prop:safety-condition} and to improve the efficiency of verification. Our observation [appendix] shows that the runtime of the verifier is majorly determined by the number of hyperplanes and hinges. The regularizer effectively limits the number of boundary hyperplanes and hinges to manage computational scalability challenges as neural network size and dimensionality increase.
% \sysname also uses a set of regularizers to guide the NCBF in satisfying the conditions of Proposition \ref{prop:safety-condition} and to enhance verification efficiency. As our observations in the appendix indicate, the verifier's runtime is primarily influenced by the number of hyperplanes and hinges. The regularizers effectively limit the number of boundary hyperplanes and hinges, addressing the computational scalability challenges that arise as neural network size and dimensionality increase.
% \sysname balancing the roles of regularizers and counterexamples by utilizing a set of coarser to finer guide during training and a counterexample-guided training with categorical profiling. 
% Furthermore, \sysname balances the roles of regularizers and counterexamples by implementing a multi-tiered guidance system during training, moving from coarser to finer granularity. This approach, combined with counterexample-guided training that includes categorical profiling, ensures targeted and effective improvements throughout the training process and hence mitigate the third challenge.


==> sections/Synthesis/VeriGuidedTraining.tex <==
\subsection{Verification Guided Synthesis}
\label{subsec:VGS}
% Verification guided training
    % Verification during training to address challenge 1 by providing a guarantee on trained NCBF. 
    % different types of CE trigger different profiles to update training to guide convergence. 
    % coarser to finer
    % CE guided training address challenge 2

% outer loop generate counterexample for the 
% calls the verifier output either true 

We first present the construction of the training dataset and the augmentation of safety counterexamples. Let $\mathcal{T}$ denote the training dataset and $\hat{x} \in \mathcal{T}$ represent a sample from the data. The initial training dataset is collected by sampling uniformly over the state space, which is typical. Given the NCBF $b_{\theta}$, the verifier checks if the conditions in Proposition \ref{prop:safety-condition} are satisfied. \sysname augments the training dataset by updating with the identified safety counterexample $\mathcal{T}\cup \{\hat{x}_{ce}\}$.  

% Let $\mathcal{T}$ denote the training dataset and $\hat{x} \in \mathcal{T}$ represent a sample from the data. The initial training dataset is collected by uniform sampling within the state space. Although uniformly distributed data play a crucial role in the initial training phase, it is not scalable to sample dense enough points near or on the boundary to effectively train the NCBF. To address this bottleneck, \sysname integrates an efficient exact verification process within the training framework to certify safety and identify safety counterexamples. Given the NCBF $b_{\theta}$, the verifier checks if the conditions in Proposition \ref{prop:safety-condition} are satisfied. If $b_{\theta}$ fails the verification, the verifier identifies safety counterexamples $\hat{x}_{ce}$ and augments the training dataset with these counterexamples $\mathcal{T}\cup \{\hat{x}_{ce}\}$. 

The verifier can identify three types of safety counterexamples based on the condition violated. 
% Correctness counterexamples, denoted by $\hat{x}_{ce}^{c}$, refers to the state that $\hat{x}_{ce}^{c} \in \mathcal{D} \cap (\mathcal{X} \setminus \mathcal{C})$. Hyperplane verification counterexamples refer to the states $\hat{x}_{ce}^{h}$ where \eqref{eq:safety-condition-2} fails.  Hinge verification counterexamples are the states $\hat{x}_{ce}^{g}$ where \eqref{eq:safety-condition-1} does not hold. 



Safety counterexamples contribute differently during the training process and should be prioritized in the following sequence: correctness, hyperplane verification, and hinge verification counterexamples. If correctness counterexamples are not properly handled, the boundary $\partial D_{\theta_i}$ is likely to shift to $\partial D_{\theta_{i+1}}$ in subsequent training epochs to meet the correctness requirements. As a result, the identified hyperplane or hinge counterexamples $\hat{x}_{ce}^{h} \in \partial D_{\theta_i}$ may not be significant since it is very likely that $\hat{x}_{ce}^{h} \notin \partial D_{\theta_{i+1}}$. Similarly, hyperplane verification counterexamples should be prioritized before hinge verification counterexamples.

% Safety counterexamples play different roles during the training process, each requiring distinct types of adjustments. Let $\hat{x}_{ce}^{c}$ denote counterexamples if $\hat{x}_{ce}^{c} \in \mathcal{D} \cap (\mathcal{X} \setminus \mathcal{C})$ referred as correctness counterexamples. Let $\hat{x}_{ce}^{h}$ and $\hat{x}_{ce}^{g}$ denote hyperplane (if \eqref{eq:safety-condition-2} fails) and hinge verification counterexamples (if \eqref{eq:safety-condition-1} fails), respectively. Correctness counterexamples may necessitate major changes in the network parameters, reflected in the boundary $\partial D$, to ensure the NCBF meets condition \eqref{eq:neural-containment} in Proposition \ref{prop:safety-condition}. Hyperplane verification counterexamples might only require minor adjustments, while hinge verification counterexamples demand careful tuning at the boundaries.

% It is essential to address different types of counterexamples at the appropriate stages of training. Prioritizing correctness counterexamples is crucial because they ensure the boundary set $\partial D_{\theta}$ is accurately defined. If correctness counterexamples are not properly handled, the boundary $\partial D_{\theta_i}$ is likely to shift to $\partial D_{\theta_{i+1}}$ in subsequent training epochs to meet the correctness requirements. As a result, the identified hyperplane or hinge counterexamples $\hat{x}_{ce}^{h} \in \partial D_{\theta_i}$ may not be significant since it is very likely that $\hat{x}_{ce}^{h} \notin \partial D_{\theta_{i+1}}$. Similarly, hyperplane verification counterexamples should be prioritized before hinge verification counterexamples. Hence, \sysname prioritizes counterexamples in the following sequence: correctness, hyperplane verification, and hinge verification counterexamples.

% \sysname further mitigates the additional computational complexity by employing a quick checking to conduct a coarser check before verification. The quick checking first uniformly samples over the state space and computes the losses $\mathcal{L}_c$ and $\mathcal{L}_c$




% \sysname balances the roles of regularizers and counterexamples by implementing a multi-tiered guidance system during training, moving from coarser to finer granularity. This approach, combined with counterexample-guided training that includes categorical profiling, ensures targeted and effective improvements throughout the training process and hence mitigate the third challenge.

% \sysname adopts 

% (ii) The integration of verifiers into the training framework leads to a significant efficiency drop due to the scalability issues of NCBF verifiers.
% (iii) Counterexample-guided training may not effectively guide the training process towards convergence. Safety counterexamples can fail to meet various conditions in Proposition \ref{prop:safety-condition}, and there is currently no systematic approach to categorize these counterexamples and provide appropriate treatments.

% Introduction to Verification-Guided Synthesis:

% Importance of integrating verification into the synthesis process.
% Overview of how verification helps in identifying and addressing safety counterexamples.
% Verifier Integration:

% Role of the verifier in the synthesis framework.
% Process of verifying the synthesized NCBF against safety conditions from Proposition 1.
% Decomposition of the verification problem into linear and nonlinear programming tasks.
% Handling Counterexamples:

% Method of generating and using counterexamples when safety violations are detected.
% Feedback loop where counterexamples improve the NCBF iteratively.
% Computational Efficiency:

% Challenges of integrating a verifier into the synthesis process.
% Strategies to mitigate computational challenges, including efficient verification methods.
% Introduction to the multi-tiered guidance system for optimizing training efficiency.

% The framework consists of an verifier, regularizer and counterexample guided training. \sysname adopts an efficient exact verifier to ensure the synthesized $b_{\theta}(x)$ meets the rigorous safety conditions in Proposition \ref{prop:safety-condition} to address the first challenge. The verifier utilize the piecewise linear characteristic of the ReLU NCBF, decompose the verification problem into linear and nonlinear programming problems and efficiently certify or identify safety counterexamples. The benefit of an efficient verifier mitigate the scalability issue in the second challenge. 
% To address the first challenge, \sysname employs an efficient exact verifier to ensure that the synthesized $b_{\theta}(x)$ meets the rigorous safety conditions outlined in Proposition \ref{prop:safety-condition}. The verifier leverages the piecewise linear nature of the ReLU NCBF and decomposes the verification problem into linear and nonlinear programming tasks. This method efficiently certifies safety or identifies counterexamples, thereby mitigating the scalability issues highlighted in the second challenge.
% \sysname leverages a set of regularizers to guide the NCBF to satisfy conditions in Proposition \ref{prop:safety-condition} and to improve the efficiency of verification. Our observation [appendix] shows that the runtime of the verifier is majorly determined by the number of hyperplanes and hinges. The regularizer effectively limits the number of boundary hyperplanes and hinges to manage computational scalability challenges as neural network size and dimensionality increase.
% \sysname also uses a set of regularizers to guide the NCBF in satisfying the conditions of Proposition \ref{prop:safety-condition} and to enhance verification efficiency. As our observations in the appendix indicate, the verifier's runtime is primarily influenced by the number of hyperplanes and hinges. The regularizers effectively limit the number of boundary hyperplanes and hinges, addressing the computational scalability challenges that arise as neural network size and dimensionality increase.
% \sysname balancing the roles of regularizers and counterexamples by utilizing a set of coarser to finer guide during training and a counterexample-guided training with categorical profiling. 
% Furthermore, \sysname balances the roles of regularizers and counterexamples by implementing a multi-tiered guidance system during training, moving from coarser to finer granularity. This approach, combined with counterexample-guided training that includes categorical profiling, ensures targeted and effective improvements throughout the training process and hence mitigate the third challenge.


% \textbf{Safety Assurance}: Ensure that $ b_{\theta}(x) $ consistently maintains system states within the safe set $ \mathcal{C} $, satisfying all derived safety conditions.

% Theoretical Objectives
% \begin{itemize}
%   \item \textbf{Safety Assurance}: Ensure that $ b_{\theta}(x) $ consistently maintains system states within the safe set $ \mathcal{C} $, satisfying all derived safety conditions.
%   \item \textbf{Verification Readiness}: Synthesize $ b_{\theta}(x) $ to inherently meet the conditions necessary for passing the adapted verification processes.
%   \item \textbf{Optimization and Efficiency}: Optimize $ b_{\theta}(x) $ to balance performance with computational efficiency, particularly focusing on scalability in larger networks.
% \end{itemize}



==> sections/Verification.tex <==
\section{Problem Formulation and Safety Conditions}
\label{sec:safety_conditions}
%In this section, we propose a framework to provide neccessary and sufficient conditions for verifying NCBF as described in Problem \ref{prob:NCBF_veri}. 
In this section, we first formally define the problem, and then give necessary and sufficient conditions for verifying NCBFs.

\subsection{Problem Formulation}
We consider a feedforward neural network (NN) $b: \mathcal{X} \rightarrow \mathbb{R}$ with ReLU activation function. Since $b$ is not continuously differentiable due to the piecewise linearity of the ReLU function, the guarantees of Theorem \ref{theorem:CBF-safety} cannot be applied directly. Our overall goal will be to derive analogous conditions to (\ref{eq:CBF-def}) for ReLU-NCBFs, and then ensure that any control policy $\mu$ that satisfies the conditions will be safe with $\mathcal{D} = \{x : b(x) \geq 0\}$.

%Our overall goal will be to ensure that, if a control policy $\mu$ satisfies (\ref{eq:CBF-def}) for this choice of $b$ for all time $t$, then $\mu$ is safe with set $\mathcal{D} = \{x : b(x) \geq 0\}$. 

%From Definition \ref{def:safe-control-policy}, this requires verifying two criteria, namely, $\mathcal{D} \subseteq \mathcal{C}$, which we denote as \emph{correctness}, and the existence of a control input $u \in \mathcal{U}$ satisfying (\ref{eq:CBF-def}) for all $x \in \mathcal{D}$, which we denote as \emph{feasibility}. 



%A CBF-based control policy may fail to guarantee safety for two reasons. First, there may exist some $x$ on the boundary of $\mathcal{D}$ such that there is no $u \in \mathcal{U}$ satisfying (\ref{eq:CBF-def}), causing the system to leave the safe region regardless of the control input that is provided. Second, there may be overlap between $\mathcal{D}$ and one of the unsafe regions, leading to safety violations even if $b(x(t)) \geq 0$ is satisfied for all time $t$. We name these two factor as feasibility and correctness, respectively. A valid CBF is required to be feasible and correct. The verification problem is even more challenging when $b(x)$ is a neural network with some non-differentiable activation functions, such as ReLU function $ReLU(z) = \max\{0,z\}$. 

\begin{problem}
\label{prob:NCBF_veri}
Given a nonlinear continuous-time system (\ref{eq:dynamics}), a neural network function $b: \mathcal{X} \rightarrow \mathbb{R}$, a set of admissible control inputs $\mathcal{U} = \{u: Au \leq c\}$ for given matrix $A \in \mathbb{R}^{p \times m}$ and vector $c \in \mathbb{R}^{p}$, and a safe set $\mathcal{C} = \{x: h(x) \geq 0\}$, determine whether (i) $\mathcal{D} \subseteq \mathcal{C}$ and (ii) there exists a control policy $\mu$ such that $\mathcal{D}$ is positive invariant  under dynamics (\ref{eq:dynamics}) and control policy $\mu$. 
\end{problem}

%     \State $(\mathcal{S}_{ij}, \mathcal{V}_{ij}) \leftarrow$ EnumerateSets$(x_{ij})$
%     \For{$\mathbf{S} \in \mathcal{S}_{ij}$}
%     \If{$\max{\{h_{i}(x) : x \in \mathcal{X}(\mathbf{S}), b(x) = 0\}} \geq 0$}
%     \Return{UNSAT}
%     \EndIf
%     \If{minimum value of (\ref{eq:single-set-nonlinear-prog}) is negative}
%     \Return{UNSAT}
%     \EndIf
%     \EndFor
%     \For{$\{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\} \in \mathcal{V}_{ij}$}
%     \If{minimum value of (\ref{eq:multiple-set-nonlinear-program}) is negative}
%     \Return{UNSAT}
%     \EndIf
%     \EndFor
%     \State \Return{SAT}
%     \EndProcedure
% \end{algorithmic}
% \label{alg:verification}
% \end{algorithm}

==> sections/Verification/Approach.tex <==
\subsection{Approach Overview}
\label{subsec:verification-overview}
The verification of NCBF consists of two major components, searching and verifying. 

\input{sections/Verification/Search}


==> sections/Verification/Formulation.tex <==
\subsection{Verification Problem Formulation}
\label{subsec:veri_formulation}

A CBF-based control policy may fail to guarantee safety for two reasons. First, there may exist some $x$ on the boundary of $\mathcal{D}$ such that there is no $u \in \mathbb{U}$ satisfying (\ref{eq:CBF-def}), causing the system to leave the safe region regardless of the control input that is provided. Second, there may be overlaps between $\mathcal{D}$ and one of the unsafe regions, leading to safety violations even if $b(x(t)) \geq 0$ is satisfied for all time $t$.
NBC verifies the safety of the feedback-controlled system \eqref{eq:dynamics} under some given policy $\mu(x\mid \lambda)$. The result relies on two components, the learned barrier function $b(x)$ and the given policy $\mu(x\mid \lambda)$. A failed verification may result from the synthesized function $b(x)$ or poorly designed policy $\mu$. Therefore a separate verification on function $b(x)$ is required. 
Both verifications share the same task that the function $b(x)$ is required to be verified to ensure (i) it correctly separates the safe and the unsafe region and (ii) it has correct Lie derivatives for every point $x\in \mathcal{C}$. 

We consider a feedforward neural network (NN) $b: \mathcal{X} \rightarrow \mathbb{R}$ with ReLU activation function. Since $b$ is not continuously differentiable due to the piecewise linearity of the ReLU function, the guarantees of Theorem \ref{theorem:CBF-safety} cannot be applied directly. Our overall goal will be to derive analogous conditions to (\ref{eq:CBF-def}) for ReLU-NCBFs, and then ensure that any control policy $\mu$ that satisfies the conditions will be safe with $\mathcal{D} = \{x: b(x) \geq 0\}$.

\begin{problem}
\label{prob:NCBF_veri}
Given a nonlinear continuous-time system (\ref{eq:dynamics}), a neural network function $b: \mathcal{X} \rightarrow \mathbb{R}$, a set of admissible control inputs $\mathcal{U} = \{u: Au \leq c\}$ for given matrix $A \in \mathbb{R}^{p \times m}$ and vector $c \in \mathbb{R}^{p}$, and a safe set $\mathcal{C} = \{x: h(x) \geq 0\}$, determine whether (i) $\mathcal{D} \subseteq \mathcal{C}$ and (ii) there exists a control policy $\mu$ such that $\mathcal{D}$ is positive invariant  under dynamics (\ref{eq:dynamics}) and control policy $\mu$. 
\end{problem}

The NCBF verification problem is challenging due to reasons from two aspects: exactness and scalability. The challenge in exact verification lies in the non-differentiability of the activation function ReLU. We propose an exact verification framework based on [*zhang23] to address this issue with two steps: searching and verifying. 
The scalability issue of the NCBF verification comes in three aspects: the dimension of the system, the number of layers, and the number of neurons. In what follows, we propose a linear-program-based searching algorithm utilizing the piece-wise linearity of ReLU neural networks to mitigate complexity from the number of neurons. The searching algorithm leverages the activation sets to characterize the input-output relationship of the network to alleviate the complexity of the number of layers and the dimension of the system. 



==> sections/Verification/SearchV0.tex <==
\subsection{Efficient Enumeration}

The efficient enumeration consists of the hyperplane enumeration identifying boundary hyperplanes and the hinge enumeration locating intersections of boundary hyperplanes. 
The boundary hyperplane can be characterized by activation sets $\mathbf{S}\in \mathcal{B}$ containing boundary $\partial \mathcal{D}$, which is equivalent to a complete search of $\mathcal{B}$. The enumeration consists of two steps (i) identifying the initial boundary activation set $\mathbf{S}_0\in \mathcal{B}$ and (ii) enumerating all $\mathbf{S}\in \mathcal{B}$ by breadth-first search (BFS). 

In the first step, we identify the boundary activation set $\mathbf{S}_0$ such that there exists some state $x\in \mathcal{X}(\mathbf{S}_0)$, $b(x)=0$. 
We first categorize the uniform distributed training data $\mathcal{T}$ into three types unsafe training set $\mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}:=\{\hat{x}: \hat{x}\in \mathcal{X}\setminus\mathcal{C}\}\subseteq \mathcal{T}$, buffer training set $\mathcal{T}_{\mathcal{C}\setminus\mathcal{I}}:=\{\hat{x}: \hat{x}\in \mathcal{C}\setminus\mathcal{I}\}\subseteq \mathcal{T}$ and safe training set $\mathcal{T}_\mathcal{I}:=\{\hat{x}: \hat{x}\in \mathcal{I}\}\subseteq \mathcal{T}$. 


% A set $\mathcal{D} \subseteq \mathbb{R}^n$ is \textit{path-connected} if for any two points $x, y \in S$, there exists a continuous path within $S$ that connects $x$ and $y$.
% A set $\mathcal{D} \subseteq \mathbb{R}^n$ is \textit{simply connected} if it is path-connected and every loop in $S$ can be continuously contracted to a point within $S$.

Since most control systems require continuous navigation, we assume that the $\mathcal{D}_\theta$ is simply connected. 
Given $\hat{x}_U\in \mathcal{T}_U$ and $\hat{x}_\mathcal{I}\in \mathcal{T}_\mathcal{I}$, define a line segment
\begin{equation}
    \label{eq:lineseg}
    \tilde{L} = \left\{ x \in \mathbb{R}^n \mid x = (1 - \lambda) \hat{x}_{\mathcal{X}\setminus\mathcal{C}} + \lambda \hat{x}_\mathcal{I}, \; \lambda \in [0, 1] \right\}
\end{equation}
The following lemma shows the initial boundary activation set $\mathbf{S}_0$ can always be produced as $\mathbf{S}_0=\mathbf{S}(\tilde{x})$ for some $\tilde{x}\in \tilde{L}$. 

\begin{lemma}
\label{lemma:enu_init}
    Given two sample points $\hat{x}_U\in \mathcal{T}_U$ and $\hat{x}_\mathcal{I}\in \mathcal{T}_\mathcal{I}$, draw a line segment $\tilde{L}$ to connect these two points. Then, there always exists a point $\tilde{x}\in \tilde{L}$ lie on this zero-level set of $b_{\theta}(x)$ and hence the initial boundary activation set $\mathbf{S}_0=\mathbf{S}(\tilde{x})$
\end{lemma}
% \begin{proof}
%     Since $b_{\theta}(x)$ is continuous and $b_{\theta}(\hat{x}_\mathcal{I}) > 0$ while $b_{\theta}(\hat{x}_{\mathcal{X}\setminus\mathcal{C}}) < 0$, there always exists only one point $\tilde{x}\in \tilde{L}$ such that $b_\theta(\tilde{x})=0$.
%     Now, suppose the line segment $\tilde{L}$ intersects the zero-level set of $b_{\theta}(x)$ multiple times. Let these intersection points be $ \tilde{x}_1, \tilde{x}_2, \ldots, \tilde{x}_k $, where $ b_{\theta}(\tilde{x}_i) = 0 $ for $ i = 1, 2, \ldots, k $. 
%     Given that the zero-level set of $\mathcal{D}_\theta$ is simply connected, containing no holes, any point of intersection $\tilde{x}_i$ on the line segment must lie on this zero-level set.
% \end{proof}
We omit the proof due to the space limit. Detailed proof can be found in Appendix \ref{appendix:proof_lemma_enuinit}. 

Given a state $x^{\prime}$, one can determine if $\mathbf{S}(x^{\prime})\in \mathcal{B}$ by solving a linear program checking if $\overline{W}(\mathbf{S}(x^{\prime})) x+\overline{r}(\mathbf{S}(x^{\prime}))=0$ is feasible for some $x\in \overline{\mathcal{X}}(\mathbf{S}(x^{\prime})$, referred as boundary linear program ($BoundaryLP(x^{\prime})$). 
The key idea is that one can identify $\mathbf{S}_0$ by identify any point $\hat{x}_\epsilon \in \mathcal{X}(\mathbf{S}(\tilde{x}))\cap \tilde{L}$. 
\sysname identifies the initial activation set by conducting a BoundaryLP-based binary search over sample sets $\mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}$ and $ \mathcal{T}_\mathcal{I}$ as shown in Alg. \ref{alg:identify}. The binary search terminates if $BoundaryLP(\hat{x}_\epsilon)$ is feasible. By Monte Carlo, Alg. \ref{alg:identify} can always find an initial boundary activation set $\mathbf{S}_0$. 


We next illustrate the enumeration of all activation sets along the zero-level set given an initial set $\mathbf{S}_0$. We define $\mathbf{S}_1$ to be a neighboring activation set with distance $d$ from $\mathbf{S}_0$ if the symmetric difference between $\mathbf{S}_0$ and $\mathbf{S}_1$ has size $d$. The symmetric difference between two sets $\mathbf{S}_0$ and $\mathbf{S}_1$, denoted by $\mathbf{A} \Delta \mathbf{B}$, is defined as:
$\mathbf{A} \Delta \mathbf{B} = (\mathbf{A} \setminus \mathbf{B}) \cup (\mathbf{B} \setminus \mathbf{A})$
We enumerate by identifying adjacent boundary activation sets ($d=1$) with Neural Breadth-First Search (NBFS). The NBFS 


% Although Proposition \ref{prob:NCBF_veri} separates the problem into hyperplanes and hinges verification, the scalability issue of the NCBF verification persists due to the dimension of the system, the depth of the network, and the size of the network. These factors increase the computational complexity of enumeration and the quantity to verify. 

% As shown in Table [*ref], searching takes most of the run time, when the network gets larger or the dimension increases. Therefore, a much more efficient search algorithm is critical to mitigate the computational complexity. To address the issue, we propose a searching algorithm to enumerate all boundary activation sets $\mathbf{S}$ where $x\in \{b(x)=0 \text{ for some } x\in \mathcal{X}(\mathbf{S})\}$. 

Our approach to enumerating the activation sets that intersect with the safety boundary is as follows. Starting with an initial point $x$ with $b(x) = 0$ (which we compute by searching along a line between $x_{0}$ and $U_{i}$), we find an activation set $\mathbf{S} \in \mathbf{S}(x)$. We then identify all sets $\mathbf{S}^{\prime}$ such that there exists $x \in \overline{\mathcal{X}}(\mathbf{S}) \cap \overline{\mathcal{X}}(\mathbf{S}^{\prime})$ with $b(x) = 0$; we observe that such an $x$ can be computed by solving a linear program. We then find all sets $S^{\prime\prime}$ with $\overline{\mathcal{X}}(\mathbf{S}^{\prime}) \cap \overline{\mathcal{X}}(\mathbf{S}^{\prime\prime}) \cap \{x: b(x) = 0\} \neq \emptyset$, continuing until we have enumerated all such activation sets that are connected to $x$. This procedure is described in detail in Algorithms \ref{alg:Enumerate}.34




\begin{algorithm}[h]
\caption{Enumerate Activated Sets}
\begin{algorithmic}[1]
    \State \textbf{Input:} State $x$ such that $b(x) = 0$
    \State \textbf{Output:} Set of activation sets $\mathcal{S}$ such that the connected component of the boundary containing $x$ is contained in $\bigcup_{\mathbf{S} \in \mathcal{S}}{\mathcal{X}(\mathbf{S})}$, set of activation sets with nonempty intersection $\mathcal{V}$
    \Procedure{Enumeration}{$x$}
    \State Uniformly sample $M$ points. The set $\mathcal{M}:=\{\tilde{x}_i^{0}, i\in \{1,\ldots,M\}\}$ 
    \State Conduct gradient decent to identify points $\tilde{x}_i$ such that $b(\tilde{x}_i)\in (-\epsilon, \epsilon)$ for $i\in \{1,\ldots,M\}$. 
    \State $BFS$
    \State \textbf{Return} ActivationSetHelper($\mathbf{S}$, $\{\mathbf{S}\}$, $\{\mathbf{S}\}$)
   \EndProcedure
\end{algorithmic}
\label{alg:Enumerate}
\end{algorithm}

The following result describes the completeness guarantees of Algorithm \ref{alg:Enumerate}.

\begin{proposition}
\label{prop:enumeration-complete}
Let $\mathcal{S}$ and $\mathcal{V}$ denote the output of Algorithm \ref{alg:Enumerate}. Then the connected component of $\{x: b(x) = 0\}$ containing the input $x$, denoted $D$, satisfies $D \subseteq \bigcup_{\mathbf{S} \in \mathcal{S}}{\overline{\mathcal{X}}(\mathbf{S})}$. Furthermore, if $\mathbf{S}_{1},\ldots,\mathbf{S}_{r} \in \mathcal{S}$ is complete and $\left(\bigcap_{i=1}^{r}{\overline{\mathcal{X}}(\mathbf{S}_{i})}\right) \cap \{x: b(x) = 0\} \neq \emptyset$, then $\{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\} \in \mathcal{V}$.
\end{proposition}

\begin{proof}
Suppose that $x^{\prime} \in D \setminus \left(\bigcup_{\mathbf{S} \in \mathcal{S}}{\overline{\mathcal{X}}(\mathbf{S})}\right)$. Since $D$ is connected, there exists a path $\gamma$ with $\gamma(0) = x$ and $\gamma(1)=x^{\prime}$ contained in $D$. Let $\mathbf{S}_{0}, \mathbf{S}_{1},\ldots,S_{K}$ denote a sequence of activation patterns with $\mathbf{S}_{0} \in \mathbf{S}(x)$, $\mathbf{S}_{K} \in \mathbf{S}(x^{\prime})$, and $\mathbf{S}_{0}$ equal to the set computed at Line 3 of Algorithm \ref{alg:Enumerate}. Then there exists $i \geq 2$ such that $\mathbf{S}_{i-1} \in \mathcal{S}$ and $\mathbf{S}_{i} \notin \mathcal{S}$, and there exists $t^{\prime}$ such that $\gamma(t^{\prime}) \in \overline{\mathcal{X}}(\mathbf{S}_{i-1}) \cap \overline{\mathcal{X}}(\mathbf{S}_{i}) \cap \{x: b(x) = 0\}$. We then have that $\mathbf{T}(\mathbf{S}_{i-1},\mathbf{S}_{i})$ is a subset of the set $\mathbf{T}$ computed at Line 4 of Algorithm \ref{alg:EnumerateHelper}, and hence $\mathbf{S}_{i}$ will be identified and added to $\mathcal{S}$ at Line 7 of Algorithm \ref{alg:EnumerateHelper}. 

Now, suppose that $\mathbf{S}_{1},\ldots,\mathbf{S}_{r} \in \mathcal{S}$ is complete and $\left(\bigcap_{i=1}^{r}{\overline{\mathcal{X}}_{0}(\mathbf{S}_{i})}\right) \cap \{x: b(x) = 0\} \neq \emptyset$. Let $l$ denote the first index such that Algorithm \ref{alg:EnumerateHelper} is called with $\mathbf{S}_{l}$ as input; without loss of generality, suppose $l=1$. Let $\mathbf{T} = \mathbf{T}(\mathbf{S}_{1},\ldots,\mathbf{S}_{r})$. Then $\mathbf{T}$ is a subset of of the set $T$ computed at line 4 of the algorithm, and the sets $\mathbf{S}_{1},\ldots,\mathbf{S}_{r}$ are enumerated at lines 7-13. Since the intersection of the $\overline{\mathcal{X}}(\mathbf{S})$ sets with $\{x: b(x) = 0\}$ is nonempty, $\{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\}$ is added to $\mathcal{V}$. 
\end{proof}





==> sections/Verification/SearchV1.tex <==
\subsection{Enumeration of Hyperplanes and Hinges}

The efficient enumeration consists of the hyperplane enumeration identifying boundary hyperplanes and the hinge enumeration locating intersections of boundary hyperplanes. 
The boundary hyperplane can be characterized by activation sets $\mathbf{S}\in \mathcal{B}$ containing boundary $\partial \mathcal{D}$, which is equivalent to a complete search of $\mathcal{B}$. The enumeration consists of two steps (i) identifying the initial boundary activation set $\mathbf{S}_0\in \mathcal{B}$ and (ii) enumerating all $\mathbf{S}\in \mathcal{B}$ by breadth-first search (BFS). 

In the first step, we identify the boundary activation set $\mathbf{S}_0$ such that there exists some state $x\in \mathcal{X}(\mathbf{S}_0)$, $b(x)=0$. 
We first categorize the uniform distributed training data $\mathcal{T}$ into three types unsafe training set $\mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}:=\{\hat{x}: \hat{x}\in \mathcal{X}\setminus\mathcal{C}\}\subseteq \mathcal{T}$, buffer training set $\mathcal{T}_{\mathcal{C}\setminus\mathcal{I}}:=\{\hat{x}: \hat{x}\in \mathcal{C}\setminus\mathcal{I}\}\subseteq \mathcal{T}$ and safe training set $\mathcal{T}_\mathcal{I}:=\{\hat{x}: \hat{x}\in \mathcal{I}\}\subseteq \mathcal{T}$. 

Since most control systems require continuous navigation, we assume that the $\mathcal{D}_\theta$ is simply connected. 
Given $\hat{x}_U\in \mathcal{T}_U$ and $\hat{x}_\mathcal{I}\in \mathcal{T}_\mathcal{I}$, define a line segment
\begin{equation}
    \label{eq:lineseg}
    \tilde{L} = \left\{ x \in \mathbb{R}^n \mid x = (1 - \lambda) \hat{x}_{\mathcal{X}\setminus\mathcal{C}} + \lambda \hat{x}_\mathcal{I}, \; \lambda \in [0, 1] \right\}
\end{equation}
The following lemma shows the initial boundary activation set $\mathbf{S}_0$ can always be produced as $\mathbf{S}_0=\mathbf{S}(\tilde{x})$ for some $\tilde{x}\in \tilde{L}$. 

\begin{lemma}
\label{lemma:enu_init}
    Given two sample points $\hat{x}_U\in \mathcal{T}_U$ and $\hat{x}_\mathcal{I}\in \mathcal{T}_\mathcal{I}$, draw a line segment $\tilde{L}$ to connect these two points. Then, there always exists a point $\tilde{x}\in \tilde{L}$ lie on this zero-level set of $b_{\theta}(x)$ and hence the initial boundary activation set $\mathbf{S}_0=\mathbf{S}(\tilde{x})$
\end{lemma}
We omit the proof due to the space limit. Detailed proof can be found in Appendix \ref{appendix:proof_lemma_enuinit}. 

Given a state $x^{\prime}$, one can determine if $\mathbf{S}(x^{\prime})\in \mathcal{B}$ by solving a linear program checking if $\overline{W}(\mathbf{S}(x^{\prime})) x+\overline{r}(\mathbf{S}(x^{\prime}))=0$ is feasible for some $x\in \overline{\mathcal{X}}(\mathbf{S}(x^{\prime})$, referred as boundary linear program ($\text{BoundaryLP}(\mathbf{S}(x^{\prime}))$) defined as follows. 
\begin{equation}
\label{eq:boundarylp}
    \text{BoundaryLP}(\mathbf{S}(x^{\prime})) = 
    \begin{cases}
    \text{find} & x \\
    \text{s.t.} & \overline{W}(\mathbf{S}(x^{\prime})) x + \overline{r}(\mathbf{S}(x^{\prime})) = 0 \\
                    & x \in \overline{\mathcal{X}}(\mathbf{S}(x^{\prime}))
    \end{cases}
\end{equation}

The key idea is that one can identify $\mathbf{S}_0$ by identify any point $\hat{x}_\epsilon \in \mathcal{X}(\mathbf{S}(\tilde{x}))\cap \tilde{L}$. 
\sysname identifies the initial activation set by conducting a BoundaryLP-based binary search over sample sets $\mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}$ and $ \mathcal{T}_\mathcal{I}$ as shown in Alg. \ref{alg:identify}. The binary search terminates if $BoundaryLP(\hat{x}_\epsilon)$ is feasible. By Monte Carlo, Alg. \ref{alg:identify} can always find an initial boundary activation set $\mathbf{S}_0$. 

We define $\mathbf{S}_1$ to be a neighboring activation set with distance $d$ from $\mathbf{S}_0$ if the symmetric difference between $\mathbf{S}_0$ and $\mathbf{S}_1$ has size $d$. The symmetric difference between two sets $\mathbf{S}_0$ and $\mathbf{S}_1$, denoted by $\mathbf{A} \Delta \mathbf{B}$, is defined as:
$\mathbf{A} \Delta \mathbf{B} = (\mathbf{A} \setminus \mathbf{B}) \cup (\mathbf{B} \setminus \mathbf{A})$

Next, we illustrate Neural Breadth-First Search (NBFS) for enumerating all activation sets along the zero-level set, given an initial set $\mathbf{S}_0$. NBFS identifies adjacent boundary activation sets ($d=1$) by the following two steps. 

\textbf{Step 1:} Given a set $\mathbf{S}$, NBFS flips one activation at a time $(i,j) \in \mathbf{S}$ to form a new neighbor $\mathbf{S}^{\prime}$ by either including $\mathbf{S}^{\prime}=\mathbf{S}\cup \{(i,j)\}$ or excluding $\mathbf{S}^{\prime}=\mathbf{S}\setminus\{(i,j)\}$. NBFS identifies the activation $(i,j)$ to flip by checking if $\overline{W}(\mathbf{S}) x+\overline{r}(\mathbf{S})=0$ is feasible for some $x\in \overline{\mathcal{X}}(\mathbf{S})\cap\{x: W_{ij}x+r_{ij}=0\}$, referred as unstable neuron linear program of $\text{USLP}(\mathbf{S}, (i,j))$ defined as follows. To further improve efficiency, we utilize hypercube $\mathcal{H}(\mathbf{S})$ to approximate $\overline{\mathcal{X}}(\mathbf{S})$.  
 
\begin{equation}
\label{eq:boundarylp}
    \text{USLP}(\mathbf{S}, (i,j)) = 
    \begin{cases}
    \text{find} & x \\
    \text{s.t.} & \overline{W}(\mathbf{S}) x + \overline{r}(\mathbf{S}) = 0 \\
                    & W_{i,j} x + r_{i,j}=0 \\
                    & x \in \mathcal{H}(\mathbf{S})
    \end{cases}
\end{equation}
\textbf{Step 2:} NBFS then determines if the new neighbor is on the boundary by checking the feasibility of $BoundaryLP(\mathbf{S}^{\prime})$.
This process continues in a breadth-first search manner until all such activation sets on the zero-level set have been enumerated and output set $\mathcal{S}$. Detailed procedure is described in Algorithm \ref{alg:NBFS}. 

Finally, we enumerate all hinges by solving the hinge linger program, referred as $\text{HingeLP}(\mathcal{S}_i)$, given a set of activation sets $\mathcal{S}_i\subseteq \mathcal{S}$. 
\begin{equation}
\label{eq:hingelp}
    \text{HingeLP}(\mathcal{S}_i) = 
    \begin{cases}
    \text{find} & x \\
    \text{s.t.} & \overline{W}(\mathbf{S}) x + \overline{r}(\mathbf{S}) = 0, \quad \forall \mathbf{S}\in \mathcal{S}_i\\
                & x \in \mathcal{X}(\mathbf{S}), \quad \forall \mathbf{S}\in \mathcal{S}_i
    \end{cases}
\end{equation}
To ensure completeness, \sysname enumerates all hinges $\mathbf{V}\in \mathcal{V}$ with $\|\mathcal{S}_i\|\in\{2, 3, \ldots, n\}$ with Algorithm \ref{alg:hinge_search}.  

\begin{algorithm}[h]
\caption{Enumerate Activated Sets}
\begin{algorithmic}[1]
    \State \textbf{Input:} $n, \mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}, \mathcal{T}_\mathcal{I}$
    \State \textbf{Output:} Set of activation sets $\mathcal{S}$, set of activation sets with nonempty intersection $\mathcal{V}$
    \Procedure{Enumeration}{$\mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}, \mathcal{T}_\mathcal{I}$}
    \State $\mathbf{S}_0 \gets \text{ENUMINIT}(\mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}, \mathcal{T}_\mathcal{I})$
    \State $\mathcal{S} \gets \text{NBFS}(\mathbf{S}_0)$
    \State $\mathcal{V} \gets \text{HingeEnum}(\mathcal{S}, n)$
    \State \textbf{Return} $\mathcal{S}$, $\mathcal{V}$
   \EndProcedure
\end{algorithmic}
\label{alg:Enumerate}
\end{algorithm}

The following result describes the completeness guarantees of Algorithm \ref{alg:Enumerate}.

\begin{proposition}
\label{prop:enumeration-complete}
Let $\mathcal{S}$ and $\mathcal{V}$ denote the output of Algorithm \ref{alg:Enumerate}. Then the connected component of $\{x: b(x) = 0\}$ containing the input $x$, denoted $D$, satisfies $D \subseteq \bigcup_{\mathbf{S} \in \mathcal{S}}{\overline{\mathcal{X}}(\mathbf{S})}$. Furthermore, if $\mathbf{S}_{1},\ldots,\mathbf{S}_{r} \in \mathcal{S}$ is complete and $\left(\bigcap_{i=1}^{r}{\overline{\mathcal{X}}(\mathbf{S}_{i})}\right) \cap \{x: b(x) = 0\} \neq \emptyset$, then $\{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\} \in \mathcal{V}$.
\end{proposition}







==> sections/Verification/SearchV2.tex <==
\subsection{Enumeration of Hyperplanes and Hinges}

The boundary enumeration identifies the boundary hyperplanes $\mathbf{S}_0\in \mathcal{B}$. It initially identifies the initial boundary activation set $\mathbf{S}_0\in \mathcal{B}$, enumerates all $\mathbf{S}\in \mathcal{B}$ by NBFS starting from $\mathbf{S}_0$ and enumerates all hinges consisting of the intersections of hyperplanes. 

% The efficient enumeration consists of the hyperplane enumeration identifying boundary hyperplanes and the hinge enumeration locating intersections of boundary hyperplanes. 
% The boundary hyperplane can be characterized by activation sets $\mathbf{S}\in \mathcal{B}$ containing boundary $\partial \mathcal{D}$, which is equivalent to a complete search of $\mathcal{B}$. The enumeration consists of two steps (i) identifying the initial boundary activation set $\mathbf{S}_0\in \mathcal{B}$ and (ii) enumerating all $\mathbf{S}\in \mathcal{B}$ by breadth-first search (BFS). 

\textbf{Initial Activation Set: }
First, we identify the initial boundary activation set $\mathbf{S}_0$.
% We first categorize the uniform distributed training data $\mathcal{T}$ into three types unsafe training set $\mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}:=\{\hat{x}: \hat{x}\in \mathcal{X}\setminus\mathcal{C}\}\subseteq \mathcal{T}$, buffer training set $\mathcal{T}_{\mathcal{C}\setminus\mathcal{I}}:=\{\hat{x}: \hat{x}\in \mathcal{C}\setminus\mathcal{I}\}\subseteq \mathcal{T}$ and safe training set $\mathcal{T}_\mathcal{I}:=\{\hat{x}: \hat{x}\in \mathcal{I}\}\subseteq \mathcal{T}$. 
% Since most control systems require continuous navigation, we assume that the $\mathcal{D}_\theta$ is simply connected. 
Given $\hat{x}_{U}\in \mathcal{X}\setminus\mathcal{C}$ and $\hat{x}_\mathcal{I}\in \mathcal{I}$, define a line segment
\begin{equation}
    \label{eq:lineseg}
    \tilde{L} = \left\{ x \in \mathbb{R}^n \mid x = (1 - \lambda) \hat{x}_{\mathcal{X}\setminus\mathcal{C}} + \lambda \hat{x}_\mathcal{I}, \; \lambda \in [0, 1] \right\}
\end{equation}
The following lemma shows the initial boundary activation set $\mathbf{S}_0$ can always be produced as $\mathbf{S}_0=\mathbf{S}(\tilde{x})$ for some $\tilde{x}\in \tilde{L}$. 

\begin{lemma}
\label{lemma:enu_init}
    Given two sample points $\hat{x}_U\in \mathcal{X}\setminus\mathcal{C}$ and $\hat{x}_\mathcal{I}\in \mathcal{I}$, let $\tilde{L}$ denote the line segment connecting these two points. Then, there exists a point $\tilde{x}\in \tilde{L}$ with $b_{\theta}(\tilde{x})=0$. 
\end{lemma}
Lemma 1 follows from the intermediate value theorem. 
The search of the initial activation set is to choose a sequence of points $x_{1}^{0}, \ldots, x_{Z}^{0} \in \tilde{L}$. For each $x_{i}^{0}$, check if $\overline{\mathcal{X}}(\mathbf{S}(x_{i}^{0}))\cap \partial \mathcal{D}\neq \emptyset$. 
% We omit the proof due to the space limit. Detailed proof can be found in Appendix \ref{appendix:proof_lemma_enuinit}.  

Given a state $x_{i}^{0}$, one can determine if $\mathbf{S}(x_{i}^{0})\in \mathcal{B}$ by solving a linear program checking if $\overline{W}(\mathbf{S}(x_{i}^{0})) x+\overline{r}(\mathbf{S}(x_{i}^{0}))=0$ is feasible for some $x\in \overline{\mathcal{X}}(\mathbf{S}(x_{i}^{0})$, referred as boundary linear program ($\text{BoundaryLP}(\mathbf{S}(x_{i}^{0}))$) defined as follows. 
\begin{equation}
\label{eq:boundarylp}
    \text{BoundaryLP}(\mathbf{S}(x_{i}^{0})) = 
    \begin{cases}
    \text{find} & x \\
    \text{s.t.} & \overline{W}(\mathbf{S}(x_{i}^{0})) x + \overline{r}(\mathbf{S}(x_{i}^{0})) = 0 \\
                    & x \in \overline{\mathcal{X}}(\mathbf{S}(x_{i}^{0}))
    \end{cases}
\end{equation}

If $\mathcal{D}$ is simply connected, $\mathbf{S}_0$ can be identified efficiently by BoundaryLP-based binary search in Algorithm \ref{alg:identify}. 
% The key idea is that one can identify $\mathbf{S}_0$ by identify any point $\hat{x}_\epsilon \in \mathcal{X}(\mathbf{S}(\tilde{x}))\cap \tilde{L}$. 
% \sysname identifies the initial activation set by conducting a BoundaryLP-based binary search over sample sets $\mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}$ and $ \mathcal{T}_\mathcal{I}$ as shown in Alg. \ref{alg:identify}. The binary search terminates if $BoundaryLP(\hat{x}_\epsilon)$ is feasible. By Monte Carlo, Alg. \ref{alg:identify} can always find an initial boundary activation set $\mathbf{S}_0$. 

% We define $\mathbf{S}_1$ to be a neighboring activation set with distance $d$ from $\mathbf{S}_0$ if the symmetric difference between $\mathbf{S}_0$ and $\mathbf{S}_1$ has size $d$. The symmetric difference between two sets $\mathbf{A}$ and $\mathbf{B}$, denoted by $\mathbf{A} \Delta \mathbf{B}$, is defined as:
% $\mathbf{A} \Delta \mathbf{B} = (\mathbf{A} \setminus \mathbf{B}) \cup (\mathbf{B} \setminus \mathbf{A})$. 

Next, we illustrate Neural Breadth-First Search (NBFS) for enumerating all activation sets along the zero-level set, given an initial set $\mathbf{S}_0$. NBFS enumerates and outputs the collection of all boundary hyperplanes denoted as $\mathcal{S}$ by repeating the following two steps. 

\textbf{Step 1:} Given a set $\mathbf{S}$, NBFS flips one activation at a time $(i,j) \in \mathbf{S}$ to form a new neighbor $\mathbf{S}^{\prime}$ by either including $\mathbf{S}^{\prime}=\mathbf{S}\cup \{(i,j)\}$ or excluding $\mathbf{S}^{\prime}=\mathbf{S}\setminus\{(i,j)\}$. NBFS identifies the activation $(i,j)$ to flip by checking if $\overline{W}(\mathbf{S}) x+\overline{r}(\mathbf{S})=0$ is feasible for some $x\in \overline{\mathcal{X}}(\mathbf{S})\cap\{x: W_{ij}x+r_{ij}=0\}$, referred as unstable neuron linear program of $\text{USLP}(\mathbf{S}, (i,j))$ defined as follows. To further improve efficiency, we overapproximate the boundary hyperplane with hypercube to $\mathcal{H}(\mathbf{S})\supseteq \overline{\mathcal{X}}(\mathbf{S})$.  
 
\begin{equation}
\label{eq:boundarylp}
    \text{USLP}(\mathbf{S}, (i,j)) = 
    \begin{cases}
    \text{find} & x \\
    \text{s.t.} & \overline{W}(\mathbf{S}) x + \overline{r}(\mathbf{S}) = 0 \\
                    & W_{i,j} x + r_{i,j}=0 \\
                    & x \in \mathcal{H}(\mathbf{S})
    \end{cases}
\end{equation}
\textbf{Step 2:} NBFS then determines if the new neighbor is on the boundary by checking the feasibility of $BoundaryLP(\mathbf{S}^{\prime})$.
This process continues in a breadth-first search manner until all such activation sets on the zero-level set have been enumerated and output set $\mathcal{S}$. Detailed procedure is described in Algorithm \ref{alg:NBFS}. A set $\mathcal{S}$ is complete if $\mathcal{S}=\mathcal{B}$. 

Given all enumerated activation sets $\mathcal{S}$, the verifier of \sysname then enumerates hinges. Let $\mathbf{V}:=\{\mathbf{S}_i: \mathbf{S}_i\in \mathcal{B}\}$ denote the hinge intersected by hyperplane $\mathbf{S}_1,\ldots,\mathbf{S}_r$. Let $\mathcal{V}$ denote the collection of hinges to be enumerated. 
The enumeration of hinges is conducted by solving the hinge linear program, referred to as $\text{HingeLP}(\mathcal{S}_i)$, given a set of activation sets $\mathcal{S}_i\subseteq \mathcal{S}$. 
\begin{equation}
\label{eq:hingelp}
    \text{HingeLP}(\mathcal{S}_i) = 
    \begin{cases}
    \text{find} & x \\
    \text{s.t.} & \overline{W}(\mathbf{S}) x + \overline{r}(\mathbf{S}) = 0, \quad \forall \mathbf{S}\in \mathcal{S}_i\\
                & x \in \mathcal{X}(\mathbf{S}), \quad \forall \mathbf{S}\in \mathcal{S}_i
    \end{cases}
\end{equation}
The hinge enumeration is complete if there does not exist a state $x\in \bigcap_{\mathbf{S}_i=\mathbf{S}_1,\ldots,\mathbf{S}_r}{\overline{\mathcal{X}}(\mathbf{S}_i)}$ such that $\{\mathbf{S}_1,\ldots,\mathbf{S}_r\}:=\mathbf{V}_{ce}\notin \mathcal{V}$. 
Given a complete set $\mathcal{S}=\mathcal{B}$, \sysname enumerates all hinges $\mathbf{V}\in \mathcal{V}$ with $|\mathcal{S}_i|\in\{2, 3, \ldots, n\}$ for all boundary activation set $\mathbf{S}\in\mathcal{S}$ with Algorithm \ref{alg:hinge_search} to ensure completeness.  

\begin{algorithm}[h]
\caption{Enumerate Activated Sets}
\begin{algorithmic}[1]
    \State \textbf{Input:} $n, \mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}, \mathcal{T}_\mathcal{I}$
    \State \textbf{Output:} Set of activation sets $\mathcal{S}$, set of activation sets with nonempty intersection $\mathcal{V}$
    \Procedure{Enumeration}{$\mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}, \mathcal{T}_\mathcal{I}$}
    \State $\mathbf{S}_0 \gets \text{ENUMINIT}(\mathcal{T}_{\mathcal{X}\setminus\mathcal{C}}, \mathcal{T}_\mathcal{I})$
    \State $\mathcal{S} \gets \text{NBFS}(\mathbf{S}_0)$
    \State $\mathcal{V} \gets \text{HingeEnum}(\mathcal{S}, n)$
    \State \textbf{Return} $\mathcal{S}$, $\mathcal{V}$
   \EndProcedure
\end{algorithmic}
\label{alg:Enumerate}
\end{algorithm}

The following result describes the completeness guarantees of Algorithm \ref{alg:Enumerate}.

\begin{proposition}
\label{prop:enumeration-complete}
Let $\mathcal{S}$ and $\mathcal{V}$ denote the output of Algorithm \ref{alg:Enumerate}. Then the connected component of $\{x: b(x) = 0\}$ containing the input $x$, denoted $D$, satisfies $D \subseteq \bigcup_{\mathbf{S} \in \mathcal{S}}{\overline{\mathcal{X}}(\mathbf{S})}$. Furthermore, if $\mathbf{S}_{1},\ldots,\mathbf{S}_{r} \in \mathcal{S}$ is complete and $\left(\bigcap_{i=1}^{r}{\overline{\mathcal{X}}(\mathbf{S}_{i})}\right) \cap \{x: b(x) = 0\} \neq \emptyset$, then $\{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\} \in \mathcal{V}$.
\end{proposition}







==> sections/Verification/VerifierV0.tex <==
\subsection{Efficient Verification}

The verification of \sysname first enumerates all boundary activation sets and hinges by employing Algorithm \ref{alg:Enumerate} and adopts exact verification to verify enumerated hyperplanes $\mathbf{S}\in\mathcal{S}$ and hinges $\mathbf{V}\in\mathcal{V}$. Verifying these conditions in Proposition \ref{prop:safety-condition} may involve solving nonlinear programs (NLPs), which are challenging for identifying global minima. 
To ensure NLPs are solved with global minima, the verification of \sysname formulates the NLP as a UNSAT problem to be solved by dReal \cite{gao2013dreal}. The following theorem shows the verification ensures $b_{\theta}(x)$ is a valid NCBF if verification is passed. 

\begin{theorem}
\label{th:verification_guarantee}
Given a NCBF $b_{\theta}(x)$, $b_{\theta}(x)$ is a valid NCBF if it passes the verification of \sysname adopting Algorithm \ref{alg:Enumerate} and dReal.
\end{theorem}
\begin{proof}
    By Lemma \ref{lemma:enu_init}, the initial boundary activation set $\mathbf{S}_0$ is ensured to be identified by the verification of \sysname in Line 4 Algorithm. \ref{alg:Enumerate}. 
    Given $\mathbf{S}_0$ and the enumeration in Line 5 and 6 Algorithm. \ref{alg:Enumerate} being complete, the completeness of $\mathcal{S}$ and $\mathcal{V}$ is guaranteed by Proposition \ref{prop:enumeration-complete}. 
    By dReal solving the equivalent NLPs, the conditions of Proposition \ref{prop:safety-condition}, are satisfied. Therefore, $b_{\theta}(x)$ is a valid NCBF
\end{proof}

We highlight that the solving time of dReal is tractable, given that the number of variables is $n$ for hyperplane verification and $n+2m$ for hinge verification. To further enhance efficiency, we introduce progressive verification conditions. The progressive verification condition consists of a type-driven sequence and a solver-driven sequence. 

Based on efficiency considerations, the verification should be prioritized based on the difficulties of identifying different types of counterexamples. Correctness counterexamples are relatively easy to be identified. They can be identified by sample-based quick checking or convex programs in each hyperplane if the given $h(x)$ are convex. Hyperplane verification requires more effort for nonlinear systems. Hinge verification consumes more computational resources, due to extra enumeration of hinges and verifications. 

The solver-driven sequence priorities conditions expedite the verification process by applying sufficient condition verification before invoking NLP or SMT solvers. A detailed guide table can be found in the [appendix].

==> sections/Verification/VerifierV1.tex <==
\subsection{Efficient Verification}
\label{subsec:efficient_veri}

The verification of \sysname first enumerates all boundary activation sets and hinges by employing Algorithm \ref{alg:Enumerate} and adopts exact verification to verify enumerated hyperplanes $\mathbf{S}\in\mathcal{S}$ and hinges $\mathbf{V}\in\mathcal{V}$. Verifying these conditions in Proposition \ref{prop:safety-condition} may involve solving nonlinear programs (NLPs), which are challenging for identifying global minima. 
To ensure NLPs are solved with global minima, the verification of \sysname formulates the NLP as a UNSAT problem to be solved by dReal \cite{gao2013dreal}. The following theorem shows the verification ensures $b_{\theta}(x)$ is a valid NCBF if verification is passed. 

\begin{theorem}
\label{th:verification_guarantee}
Given a NCBF $b_{\theta}(x)$, $b_{\theta}(x)$ is a valid NCBF if it passes the verification of \sysname adopting Algorithm \ref{alg:Enumerate} and dReal.
\end{theorem}
\begin{proof}
    By Lemma \ref{lemma:enu_init}, the initial boundary activation set $\mathbf{S}_0$ is ensured to be identified by the verification of \sysname in Line 4 Algorithm. \ref{alg:Enumerate}. 
    Given $\mathbf{S}_0$ and the enumeration in Line 5 and 6 Algorithm. \ref{alg:Enumerate} being complete, the completeness of $\mathcal{S}$ and $\mathcal{V}$ is guaranteed by Proposition \ref{prop:enumeration-complete}. 
    By dReal solving the equivalent NLPs, the conditions of Proposition \ref{prop:safety-condition}, are satisfied. Therefore, $b_{\theta}(x)$ is a valid NCBF
\end{proof}

We highlight that the solving time of dReal is tractable, given that the number of variables is $n$ for hyperplane verification and $n+2m$ for hinge verification. To further enhance efficiency, we introduce progressive verification conditions. The progressive verification condition consists of a type-driven sequence and a solver-driven sequence. 

Based on efficiency considerations, the verification should be prioritized based on the difficulties of identifying different types of counterexamples. Correctness counterexamples are relatively easy to be identified. They can be identified by sample-based quick checking or convex programs in each hyperplane if the given $h(x)$ are convex. Hyperplane verification requires more effort for nonlinear systems. Hinge verification consumes more computational resources, due to extra enumeration of hinges and verifications. 

The solver-driven sequence priorities conditions expedite the verification process by applying sufficient condition verification before invoking NLP or SMT solvers. A detailed guide table can be found in the [appendix].

==> sections/Verification/VerifierV2.tex <==
\subsection{Efficient Verification}
\label{subsec:efficient_veri}

% We verify in the sequence of difficulties, correctness, hyperplanes, hinges. Embed into search for quick exit or early stop
%Given the set of boundary hyperplanes $\mathcal{S}$ and the set of boundary hinges $\mathcal{V}$, we verify the satisfaction of condition in Proposition \ref{prop:safety-condition} in three aspects. The proposed verification certifies the correctness (\eqref{eq:neural-containment} in condition (ii)) and hyperplane condition (\eqref{eq:safety-condition-2} in condition (i)) for each activation set $\mathbf{S}\in\mathcal{S}$. The verification certifies each hinge $\mathbf{V}\in \mathcal{V}$ to check if \eqref{eq:safety-condition-1}-\eqref{eq:safety-condition-2} in condition (i) hold.

The efficient verification component takes the sets of boundary hyperplanes $\mathcal{S}$ and boundary hinges $\mathcal{V}$ and checks that the conditions of Proposition \ref{prop:safety-condition} hold for each of them. As pointed out after Proposition \ref{prop:safety-condition}, the problem of searching for safety counterexamples can be decomposed into searching for correctness, hyperplane, and hinge counterexamples. In order to maximize the efficiency of our approach, we first consider the least computationally burdensome verification task, namely, searching for correctness counterexamples. We then search for hyperplane counterexamples, followed by hinge counterexamples.
%These search problems have varying complexities; in our experiments, correctness was typically the easiest to verify, followed by searching for hyperplane counterexamples, and searching for hinge counterexamples was the most challenging. 


%Based on efficiency considerations, the verification should be prioritized based on the difficulties with the sequence of correctness, hyperplane, and hinge verification, as shown in Algorithm \ref{alg:EEV}. 
%In what follows, we detail the verification in each aspect with sufficient conditions to improve efficiency. We note that most of the cases can be efficiently handled by sufficient condition verification. 

\textbf{Correctness Verification: }
% Correctness: (i) NLP as the general case (ii) LP or CVX can be adopted
The correctness condition (\eqref{eq:neural-containment}) can be verified for boundary hyperplane $\overline{\mathcal{X}}(\mathbf{S})$ by solving the  nonlinear program
\begin{equation}
\label{eq:containment-verification}
\begin{array}{ll}
\min_x & h(x) \\
\mbox{s.t.} & \overline{W}(\mathbf{S})^{T}x + \overline{r}(\mathbf{S}) = 0, x \in \overline{\mathcal{X}}
(\mathbf{S})
\end{array}
\end{equation}
When $h(x)$ is convex, \eqref{eq:containment-verification} can be solved efficiently. Otherwise, dReal can be used to check satisfiability of \eqref{eq:containment-verification} in a tractable runtime.

%We ensure the correctness of general cases by leveraging dReal to check UNSAT. The solving time of dReal is tractable even for the worst case due to a small number of variables to be solved, i.e., $x\in \mathbb{R}^n$. 
%The problem relaxes to a convex optimization when $h(x)$ is convex, which still provides an exact verification.   

\textbf{Hyperplane Verification: } 
% Hyperplane: (i) NLP as the general case (ii) Sufficient conditions (interval and no constraint) (iii) LP or CVX can be more efficient.
Hyperplane counterexamples can be identified by solving the optimization problem
\begin{equation}
    \label{eq:hyperplane-verification-exact}
    \begin{array}{ll}
    \mbox{min}_{x} & \max{\{\overline{W}(\mathbf{S})^{T}(f(x)+g(x)u): u \in \mathcal{U}\}} \\
    \mbox{s.t.}& \overline{W}(\mathbf{S})^{T}x + \overline{r}(\mathbf{S}) = 0,  x \in \overline{\mathcal{X}}(\mathbf{S})
     \end{array}
\end{equation}
%The hyperplane condition can be certified by solving the nonlinear program in Appendix \ref{appendix:verification:hyperplan_verification}. 

Solving \eqref{eq:hyperplane-verification-exact} can be made more efficient when additional structures on the input set $\mathcal{U}$ and dynamics $f$ and $g$ are present. Consider a case $\mathcal{U} = \{D\omega : ||\omega||_{\infty} \leq 1\}$. In this case, the problem reduces to the  nonlinear program 
\begin{equation}
\begin{split}
\label{eq:interval_minLf}
    \min_x  \quad & \overline{W}(\mathbf{S})^{T} f(x) + \|\overline{W}(\mathbf{S}) g(x) D \|_1 \\
    \text{s.t.} \quad & \overline{W}(\mathbf{S})^{T} x + \overline{r}(\mathbf{S}) = 0,
                x \in \overline{\mathcal{X}}(\mathbf{S})
\end{split}
\end{equation}
If $f(x)$ and $g(x)$ are linear in $x$, then the problem boils down to a linear program. If bounds on the Lipschitz coefficients of $f$ and $g$ are available, then they can be used to derive approximations of \eqref{eq:interval_minLf}.

If $\mathcal{U} = \mathbb{R}^{m}$, then  by \cite[Corollary 1]{zhang2023exact}, the problem can be reduced to the  nonlinear program 
\begin{equation}
\label{eq:single-set-nonlinear-prog-special-case}
\begin{array}{ll} 
\min_{x} & \overline{W}(\mathbf{S})^{T}f(x) \\
\mbox{s.t.} 
& \overline{W}(\mathbf{S})^{T}g(x) = 0, \overline{W}(\mathbf{S})x + \overline{r}(\mathbf{S}) = 0, x \in \overline{\mathcal{X}}
(\mathbf{S}) 
\end{array}
\end{equation}
If $g(x)$ is a constant matrix $G$, then safety is automatically guaranteed if $\overline{W}(\mathbf{S})^{T}G \neq 0$. If $f(x)$ is linear in $x$ as well, then (\ref{eq:single-set-nonlinear-prog-special-case}) is a linear program. 

\textbf{Hinge Verification: }
% Hinge: (i) NLP as the general case (ii) sufficient conditions (iii) early stop in searching
%The hinge can be certified by checking the conditions in \cite[Lemma 4]{zhang2023exact}. 
The hinge $\mathbf{V} = \{\mathbf{S}_{1},\ldots,\mathbf{S}_{r}\}$ can be certified by solving the nonlinear optimization problem
\begin{equation}
    \label{eq:hinge-certify}
    \begin{array}{ll}
    \mbox{min}_{x} & \max{\{\overline{W}(\mathbf{S}_{l})^{T}(f(x)+g(x)u) : l=1,\ldots,r, u \mbox{ satisfies \eqref{eq:safety-condition-1}--\eqref{eq:safety-condition-1a}}\}} \\
    \mbox{s.t.} & x \in \overline{\mathcal{X}}(\mathbf{S}_{1}) \cap \cdots \cap \overline{\mathcal{X}}(\mathbf{S}_{r}), \overline{W}(\mathbf{S}_{1})^{T}x + \overline{r}(\mathbf{S}_{1}) = 0
    \end{array}
\end{equation}
In practice, simple heuristics are often sufficient to verify safety of hinges without resorting to solving \eqref{eq:hinge-certify}. If $\overline{W}(\mathbf{S})^{T}f(x) > 0$ for all $x \in \overline{\mathcal{X}}(\mathbf{S}_{1}) \cap \cdots \cap \overline{\mathcal{X}}(\mathbf{S}_{r})$, then the control input $u = \mathbf{0}$ suffices to ensure safety. Furthermore, if $\mathcal{U} = \mathbb{R}^{m}$ and there exists $i \in \{1,\ldots,m\}$ and $s \in \{0,1\}$ such that $\mbox{sign}((\overline{W}(\mathbf{S}_{l})^{T}g(x))_{i}) = s$ for all $x \in \overline{\mathcal{X}}(\mathbf{S}_{1}) \cap \cdots \overline{\mathcal{X}}(\mathbf{S}_{r})$ and $l=1,\ldots,r$, then $u$ can be chosen as $u_{i} = Ks$ for some sufficiently large $K > 0$ to ensure that the conditions of Proposition \ref{prop:safety-condition}.


%We note that it is a lot more efficient to show the existence of $u$. 
%Consider verifying a hinge $\mathbf{V}=\{\mathbf{S}_1, \ldots, \mathbf{S}_r\}$ of $r$ hyperplanes.
%It suffices to show there exists at least a solution $u=\mathbb{0}^{m}$ if the optimal value of the $\min_x \overline{W}(\mathbf{S})f(x)$ is positive for all $\mathbf{S}\in \mathbf{V}$. We note that this simple sufficient condition can help enhance the efficiency of the hinge enumerations in Section \ref{subsec:enumeration}. The key is that if the hinge is surrounded by hyperplanes with $\overline{W}(\mathbf{S})f(x)\geq 0$, then there automatically exists a control input $u=\mathbf{0}^m$. 
%For the cases with $g(x)=G$ without control constraints, there exists a control input if $\overline{W}(\mathbf{S})G$ share the same sign for all $\mathbf{S}\in \mathbf{V}$. 

%\textbf{Sample-based Quick Check: } To minimize the 
% \begin{equation}
%     \label{eq:hinge_Lf_min}
%     \min_x  \quad & \overline{W}(\mathbf{S}) f(x) \\
%     \text{s.t.} \quad & \overline{W}(\mathbf{S}) x + \overline{r}(\mathbf{S}) = 0
% \end{equation}
% $\overline{W}f(x)$

\textbf{Safety Guarantee: } The safety guarantees of our proposed approach are summarized in Theorem \ref{th:verification_guarantee}.
% Safety guarantee
%The verification of \sysname first enumerates all boundary activation sets and hinges by with the enumeration introduced in Section \ref{subsec:enumeration} and adopts exact verification to verify enumerated hyperplanes $\mathbf{S}\in\mathcal{S}$ and hinges $\mathbf{V}\in\mathcal{V}$. Verifying these conditions in Proposition \ref{prop:safety-condition} may involve solving nonlinear programs (NLPs), which are challenging for identifying global minima. 
%To ensure NLPs are solved with global minima, the verification of \sysname formulates the NLP as a UNSAT problem to be solved by dReal \cite{gao2013dreal}. The following theorem shows the verification ensures $b_{\theta}(x)$ is a valid NCBF if verification is passed. 

\begin{theorem}
\label{th:verification_guarantee}
Given a NCBF $b_{\theta}(x)$, $b_{\theta}(x)$ is a valid NCBF if it passes the verification of  Algorithm \ref{alg:EEV} using dReal to solve the optimization problems \eqref{eq:containment-verification}, \eqref{eq:hyperplane-verification-exact}, and \eqref{eq:hinge-certify}.
\end{theorem}
\begin{proof}
    By Lemma \ref{lemma:enu_init}, the initial boundary activation set $\mathbf{S}_0$ is ensured to be identified by the verification of \sysname in Line 4 Algorithm. \ref{alg:EEV}. 
    Given $\mathbf{S}_0$ and the enumeration in Line 5 and 6 Algorithm. \ref{alg:EEV} being complete, the completeness of $\mathcal{S}$ and $\mathcal{V}$ is guaranteed by Proposition \ref{prop:enumeration-complete}. 
    By dReal solving the equivalent NLPs, the conditions of Proposition \ref{prop:safety-condition}, are satisfied. Therefore, $b_{\theta}(x)$ is a valid NCBF
\end{proof}



==> sections/timeline.tex <==

\subsection{Timeline}
\begin{itemize}
    \item (05/16) Synthesis
    \item (05/17) Verification
    \item (by 05/17) Comparison
    \item (05/18) Experiment
    \item (05/19) Related work
    \item (05/20) Intro Conclusion
    \item (by 05/22) Main Conference Paper Submission
\end{itemize}


